On the Relative Strength of Pebbling and Resolution

The last decade has seen a revival of interest in pebble games in the context of proof complexity. Pebbling has proven a useful tool for studying resolution-based proof systems when comparing the strength of different subsystems, showing bounds on proof space, and establishing size-space trade-offs. The typical approach has been to encode the pebble game played on a graph as a CNF formula and then argue that proofs of this formula must inherit (various aspects of) the pebbling properties of the underlying graph. Unfortunately, the reductions used here are not tight. To simulate resolution proofs by pebblings, the full strength of nondeterministic black-white pebbling is needed, whereas resolution is only known to be able to simulate deterministic black pebbling. To obtain strong results, one therefore needs to find specific graph families which either have essentially the same properties for black and black-white pebbling (not at all true in general) or which admit simulations of black-white pebblings in resolution. This paper contributes to both these approaches. First, we design a restricted form of black-white pebbling that can be simulated in resolution and show that there are graph families for which such restricted pebblings can be asymptotically better than black pebblings. This proves that, perhaps somewhat unexpectedly, resolution can strictly beat black-only pebbling, and in particular that the space lower bounds on pebbling formulas in [Ben-Sasson and Nordstrom 2008] are tight. Second, we present a versatile parametrized graph family with essentially the same properties for black and black-white pebbling, which gives sharp simultaneous trade-offs for black and black-white pebbling for various parameter settings. Both of our contributions have been instrumental in obtaining the time-space trade-off results for resolution-based proof systems in [Ben-Sasson and Nordstrom 2009].

==> acknowledgements.tex <==
\section*{Acknowledgements}

I would like to thank
David Carlson,
Nicholas Pippenger,
and
\mbox{John Savage}
for helpful correspondence regarding their papers on pebbling,
and 
Eli Ben-Sasson 
and 
Johan Håstad
for stimulating discussions about pebbling and proof complexity.
I am also grateful to the
\emph{CCC~'10}
anonymous referees for useful suggestions and comments.




==> definitions-article.tex <==
%
% MISCELLANEOUS DEFINITIONS TO USE IN LaTeX-FILES
%-------------------------------------------------
%
% Last updated 08-01-14
%

%
% Stuff specific for the ``article'' article class.
%

%
% EQUATIONS, THEOREMS, PROOFS AND SUCH
%
% Requires \usepackage{amstex} or \usepackage{amsmath}
% Requires \usepackage{theorem}
% Requires \usepackage{ifthen}
%

%
% To get equation numbered within sections, e.g. (3.2) for the 2nd
% equation in section 3, use \numberwithin
%\numberwithin{equation}{section}
%
% To get a cross-reference to an equation with parantheses, use
% \eqref{}
%
% To get ``subequations'' numbered e.g. (4.9a), (4.9b), use
% \begin{subequations}
%       equations to be numbered
% \end{subequations}
%

%
% NOTE THAT \theoremheaderfont{} IS A *GLOBAL* DECLARATION!
%

% number all theorem structures using ``standardlocalcounter'' 
% with consecutive numbers
\newtheorem{standardlocalcounter}{Dummy}[section]
\newtheorem{standardglobalcounter}{Dummy}

% insert a linebreak between theorem head and body
\theoremstyle{plain}    

\newtheorem{theorem}[standardlocalcounter]{Theorem}
\newtheorem{lemma}[standardlocalcounter]{Lemma}
\newtheorem{proposition}[standardlocalcounter]{Proposition}
\newtheorem{corollary}[standardlocalcounter]{Corollary}
\newtheorem{observation}[standardlocalcounter]{Observation}
\newtheorem{fact}[standardlocalcounter]{Fact}

\newtheorem{conjecturelocalcounter}[standardlocalcounter]{Conjecture}
\newtheorem{conjectureglobalcounter}[standardglobalcounter]{Conjecture}
\newtheorem{conjecture}[standardglobalcounter]{Conjecture}
\newtheorem{openquestion}[standardglobalcounter]{Open Question}
\newtheorem{openproblem}[standardglobalcounter]{Open Problem}
\newtheorem{problem}{Problem}

\theoremstyle{definition}

\newtheorem{property}[standardlocalcounter]{Property}
\newtheorem{definition}[standardlocalcounter]{Definition}
\newtheorem{claim}[standardlocalcounter]{Claim}

\theoremstyle{remark}
\newtheorem{remark}[standardlocalcounter]{Remark}
\newtheorem{example}[standardlocalcounter]{Example}


%
% STUFF FOR ``META-KIND'' OF INTERNAL NOTES --- OBSOLETE 
%

% META COMMENT
\newtheoremstyle{meta}% name
  {3pt}%      Space above
  {3pt}%      Space below
  {\scshape \small }%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape \small }% Thm head font
  {:}%        Punctuation after thm head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{meta}
\newtheorem{meta}{Meta comment}

% OPEN QUESTIONS (IN META COMMENT STYLE INTENDED FOR PRIVATE NOTES)
\newtheoremstyle{questions}% name
  {3pt}%      Space above
  {3pt}%      Space below
  {\sffamily \slshape}%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries \sffamily \slshape}% Thm head font
  {:}%        Punctuation after thm head
  { }%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{questions}
\newtheorem{questions}{Open questions}




==> doctypedetection.tex <==
%
% DETECTION OF DOCUMENT TYPE
%----------------------------
%
% Version date: March 15, 2010
%
%
% This file needs to be included or inputted so that the conditional
% macro definitions in e.g. the files definitions.tex,
% notationProofComplexity.tex, and notationClauseSpacePebbling.tex 
% will not generate compilation errors for LaTeX.
%

%
% (1)  \conference is used (rightly or wrongly) to detect poster file.
% 
% (2)  \affaddr is used (rightly or wrongly) to detect STOC file.
%     
% (3)  \affiliation and \Section} are used (rightly or wrongly) to detect 
%      FOCS file.
%     
% (4)  \conference is used (rightly or wrongly) to detect poster file.
%     
% (5)  \sicomp is used to detect SIAM journal file.
%     
% (6)  \tnotetext and \ead are used to detect Elsevier journal file.
%     
% (7)  The combination of \journal, \volume, \issue, \copyrightowner, \pubyear,
%      and \articletitle is used (rightly or wrongly) to detect NOW publishers
%      Foundations & Trends.
%     
% (8)  The combination of \keywords, \subjclass, \titlecomment, \revisionname,
%      and \lmcsheading is used (rightly or wrongly) to detect the LMCS style
%      file.
%     
% (9)  The combination of \IEEEtransversionmajor, \IEEEtransversionminor, 
%      \IEEEitemize, \IEEEenumerate, and \IEEEdescription is used (rightly
%      or wrongly) to detect IEEE style file (for CCC)
%     
% (10) If \chapter is not defined, maybeArticle is set to true.
%     
% (11) maybeThesis detects some kthesis-specific macros.
%     
% (12) maybeReport is set to true if neither maybeArticle nor maybeThesis 
%      is true.
%     
%    
% Detection of LLNCS is not implemented.
% 
%
% Use the file 'testdoctypedetection.tex' to test if these
% Boolean detectors work.
%

\usepackage{ifthen}

\newboolean{maybeSTOC}
\newboolean{maybeFOCS}
\newboolean{maybeElsevier}
\newboolean{maybeNOW}
\newboolean{maybeLMCS}
\newboolean{maybePoster}
\newboolean{maybeSIAM}
\newboolean{maybeIEEE}
\newboolean{maybeArticle}
\newboolean{maybeReport}
\newboolean{maybeThesis}

\ifthenelse{\isundefined{\affaddr}}        
{\setboolean{maybeSTOC}{false}}
{\setboolean{maybeSTOC}{true}}

\ifthenelse{\not \isundefined{\affiliation}
  \and \not \isundefined{\Section}}        
{\setboolean{maybeFOCS}{true}}
{\setboolean{maybeFOCS}{false}}

\ifthenelse{\not \isundefined{\tnotetext}
  \and \not \isundefined{\ead}}        
{\setboolean{maybeElsevier}{true}}
{\setboolean{maybeElsevier}{false}}

\ifthenelse{\not \isundefined{\journal} \and 
  \not \isundefined{\volume} \and 
  \not \isundefined{\issue} \and 
  \not \isundefined{\copyrightowner} \and 
  \not \isundefined{\articletitle} \and 
  \not \isundefined{\pubyear}}
{\setboolean{maybeNOW}{true}}
{\setboolean{maybeNOW}{false}}

\ifthenelse{\not \isundefined{\keywords} \and
  \not \isundefined{\subjclass} \and
  \not \isundefined{\titlecomment} \and
  \not \isundefined{\revisionname} \and
  \not \isundefined{\lmcsheading}}
{\setboolean{maybeLMCS}{true}}
{\setboolean{maybeLMCS}{false}}

\ifthenelse{\not \isundefined{\IEEEtransversionmajor} \and 
  \not \isundefined{\IEEEtransversionminor} \and 
  \not \isundefined{\IEEEitemize} \and 
  \not \isundefined{\IEEEenumerate} \and 
  \not \isundefined{\IEEEdescription}}
{\setboolean{maybeIEEE}{true}}
{\setboolean{maybeIEEE}{false}}

\ifthenelse{\isundefined{\sicomp}}
{\setboolean{maybeSIAM}{false}}
{\setboolean{maybeSIAM}{true}}

\ifthenelse{\isundefined{\conference}}
{\setboolean{maybePoster}{false}}
{\setboolean{maybePoster}{true}}

\ifthenelse{\isundefined{\chapter}}
{\setboolean{maybeArticle}{true}}
{\setboolean{maybeArticle}{false}}

\ifthenelse{\not \isundefined{\examen} 
  \and \not \isundefined{\disputationsdatum} 
  \and \not \isundefined{\disputationslokal}}   
  {\setboolean{maybeThesis}{true}}
  {\setboolean{maybeThesis}{false}}
           
\ifthenelse{\boolean{maybeArticle} \or \boolean{maybeThesis}}      
{\setboolean{maybeReport}{false}}
{\setboolean{maybeReport}{true}}



==> figGraphCSbasecase.tex <==
\ifthenelse{\boolean{confversionflag}}	   
{\begin{figure}[tp]
  \centering
  \includegraphics{graphCarlsonSavage.1}
  \caption{Base case for Carlson-Savage graph with $3$ spines and sinks.}
  \label{fig:graph-cs-base-case}
\end{figure}}
{\begin{figure}[tp]
  \centering
  \includegraphics{graphCarlsonSavage.1}
  \caption{Base case for Carlson-Savage graph with $3$ spines and sinks.}
  \label{fig:graph-cs-base-case}
\end{figure}}



==> figGraphCSinduction.tex <==
\ifthenelse{\boolean{confversionflag}}	   
{\begin{figure*}[tp]}
{\begin{figure}[tp]}
  \centering
  \includegraphics{graphCarlsonSavage.2}
  \caption{Inductive definition of Carlson-Savage graph $\csdag{3}{\csrec+1}$
    with $3$ spines and sinks.}
  \label{fig:graph-cs-induction}
\ifthenelse{\boolean{confversionflag}}	   
{\end{figure*}}
{\end{figure}}




==> notationClauseSpacePebbling.tex <==
%
% NOTATION USED IN PEBBLING FORMULA AND RESOLUTION SPACE RESEARCH
%-----------------------------------------------------------------
%
% AUTHOR
%
% Jakob Nordström <jakobn@kth.se>
%
% VERSION
%
% Last updated November 26, 2008
%    


% Used to get some slightly more esoteric math symbols for e.g.
% \clmentionvert and \hiddenvertices        
\usepackage{stmaryrd} 

%
% U N S O R T E D 
%-----------------
%

\newcommand{\usefulclauseadj}{useful\xspace}

\newcommand{\nclausesof}[1]{\setsize{#1}}
\newcommand{\nclausesofcompact}[1]{\setsizecompact{#1}}  % OBSOLETE
\newcommand{\Nclausesof}[1]{\Setsize{#1}}


%
% G E N E R A L   F O R M A T T I N G   R U L E S 
%-------------------------------------------------
%
% To achieve some kind of consistency in the notation
%

% MOVED TO definitions.tex
% Format of functions to integers or real numbers
%    \newcommand{\formatfunctiontonumbers}[1]{\mathrm{#1}}
%
% Format of functions to sets
%    \newcommand{\formatfunctiontoset}[1]{\mathit{#1}}
% END OF MOVED TO definitions.tex

% Format of functions to subconfigurations
\newcommand{\formatfunctiontosubconfiguration}[1]{\mathsf{#1}}
%    \newcommand{\formatfunctiontosubconfiguration}[1]{\mathrm{#1}}

%    \formatpebblingstrategy, \formatconfiguration and \formatpebblingprice 
%    are defined in notationProofComplexity.tex

%Format of functions to black multi-pebbles and white pebbles
\newcommand{\formatfunctiontomulti}[1]{\mathcal{#1}}


%    
% M I S C E L L A N E O U S   P E B B L I N G   A N D   S P A C E     
%-----------------------------------------------------------------
%

%
% SOME PEBBLING TERMINOLOGY
%
% Unconditional: starts from empty graph
% Complete: starts from empty graph and ends with (only) black on sink
% Canonical: resulting from some kind of preprocessing
%

\newcommand{\pebconditional}{conditional\xspace}
\newcommand{\Pebconditional}{Conditional\xspace}
\newcommand{\pebunconditional}{unconditional\xspace}
\newcommand{\Pebunconditional}{Unconditional\xspace}
\newcommand{\pebcomplete}{complete\xspace}
\newcommand{\Pebcomplete}{Complete\xspace}
\newcommand{\pebcompletely}{completely\xspace}
\newcommand{\Pebcompletely}{Completely\xspace}

\newcommand{\pebwellbehaved}{well-behaved\xspace}
\newcommand{\Pebwellbehaved}{Well-behaved\xspace}
\newcommand{\PEBWELLBEHAVED}{Well-Behaved\xspace}

\newcommand{\pebdominate}{dominate\xspace}
\newcommand{\pebdominationfree}{domination-free\xspace}
\newcommand{\Pebdominationfree}{Domination-free\xspace}

\newcommand{\pebnonredundant}{non-redundant\xspace}
\newcommand{\Pebnonredundant}{Non-redundant\xspace}
\newcommand{\pebredundant}{redundant\xspace}
\newcommand{\Pebredundant}{Redundant\xspace}

\newcommand{\pebfrugal}{frugal\xspace}
\newcommand{\Pebfrugal}{Frugal\xspace}
\newcommand{\pebfrugality}{frugality\xspace}
\newcommand{\Pebfrugality}{Frugality\xspace}
\newcommand{\pebnonfrugal}{non-frugal\xspace}
\newcommand{\Pebnonfrugal}{Non-frugal\xspace}
\newcommand{\pebinflationfrugal}{inflation-frugal\xspace}
\newcommand{\Pebinflationfrugal}{Inflation-frugal\xspace}

\newcommand{\pebcanonical}{canonical\xspace}
\newcommand{\Pebcanonical}{Canonical\xspace}
\newcommand{\pebintermediate}{sequence-intermediate\xspace}
\newcommand{\Pebintermediate}{Sequence-intermediate\xspace}


%    
% S P A C E   A N D   P E B B L I N G   C O M M O N   T H I N G S  
%-----------------------------------------------------------------    
%    

%
% PEBBLING FORMULA STUFF
%

\DeclareMathOperator{\dummystar}{*}
\newcommand{\pebblingcontrNT}[2][G]%
 {\ensuremath{\dummystar\!\!\formulaformat{Peb}^{#2}_{#1}}}
\newcommand{\pebcontrNT}[2][G]{\pebblingcontrNT[#1]{#2}}

% New definition using mathtools places smaller star higher up
% Does not look as pretty
%    \renewcommand{\pebcontrNT}[2][G]%
%        {\prescript{*\!\!}{}{\formulaformat{Peb}^{#2}_{#1}}}

%
% ``WITNESS'' CLAUSES
%

\newcommand{\somenodetrueclause}[1]{\formulaformat{All}^{+}\!({#1})}
% Not too good---the degree should be a supindex, not a subindex
\newcommand{\somenodetrueclausedeg}[2]{\formulaformat{All}_{#1}^{+}({#2})}


%
% CLAUSES MENTIONING VERTICES, VERTICES MENTIONED BY CLAUSES
%

\newcommand{\cmvleftdelim}{[}
\newcommand{\cmvrightdelim}{]}
\renewcommand{\cmvleftdelim}{\llbracket}
\renewcommand{\cmvrightdelim}{\rrbracket}

% OBSOLETE VARIANTS
\newcommand{\clmentionvertcompact}[2]{{#1} \bigl\cmvleftdelim {#2} \bigr\cmvrightdelim}
\newcommand{\clmentionvertsmall}[2]{{#1} \cmvleftdelim {#2} \cmvrightdelim}

% NEW VARIANTS
\newcommand{\clmentionvert}[2]{{#1} \cmvleftdelim {#2} \cmvrightdelim}
\newcommand{\Clmentionvert}[2]{{#1} \bigl\cmvleftdelim {#2} \bigr\cmvrightdelim}
\newcommand{\clposmentionvert}[2]{{#1}^{+}\!\cmvleftdelim {#2} \cmvrightdelim}
\newcommand{\clnegmentionvert}[2]{{#1}^{-}\!\cmvleftdelim {#2} \cmvrightdelim}

\newcommand{\verticespos}[1]{{\ensuremath{V^{+}\!( {#1} )}}}
\newcommand{\verticesneg}[1]{{\ensuremath{V^{-}\!( {#1} )}}}


%
% VERTICES ABOVE AND BELOW GIVEN VERTEX
%

%    \newcommand{\unrelatedverticesadj}{unrelated\xspace}
\newcommand{\unrelatedverticesadj}{non-comparable\xspace}
\newcommand{\relatedverticesadj}{comparable\xspace}

\newcommand{\crossedletter}[1]{{\times\mkern-12mu #1}}
\newcommand{\strickenletter}[1]{{-\mkern-12mu #1}}
\newcommand{\diagstrickenletter}[1]{{/\mkern-9mu #1}}
\newcommand{\slashedstrickenletter}[1]{{\backslash\mkern-9mu #1}}
            
\newcommand{\strikethroughcommand}[1]{\slashedstrickenletter{#1}}
%    \newcommand{\strikethroughcommand}[1]{\strickenletter{#1}}
%    \newcommand{\strikethroughcommand}[1]%
%    {\hspace{-0.3pt}\diagstrickenletter{#1}}
%    \newcommand{\strikethroughcommandwide}[1]{\cancel{#1}}

\newcommand{\abovevertices}[2][G]%
    {{#1}_{#2}^{\hspace{-0.2 pt}\triangledown}}
\newcommand{\aboveverticesNR}[2][G]%
    {{#1}_{\strikethroughcommand{#2}}^{\hspace{-0.3 pt}\triangledown}}
%    \newcommand{\aboveverticesNRwide}[2][G]%
%        {{#1}_{\strikethroughcommandwide{#2}}^%
%    {\hspace{-0.3 pt}\triangledown}}
%    \newcommand{\aboveverticesNR}[2][G]%
%        {{#1}_{\hspace{-0.6 pt}\strikethroughcommand{#2}}^%
%    {\hspace{-0.2 pt}\triangledown}}
\newcommand{\belowvertices}[2][G]%
    {{#1}^{#2}_{\hspace{-0.6 pt}\vartriangle}}
\newcommand{\belowverticesNR}[2][G]%
    {{#1}^{\strikethroughcommand{#2}}_{\hspace{-0.6 pt}\vartriangle}}
%    \newcommand{\belowverticesNRwide}[2][G]%
%        {{#1}^{\strikethroughcommandwide{#2}}_{\hspace{-0.6 pt}\vartriangle}}
%    \newcommand{\belowverticesNR}[2][G]%
%        {{#1}^{\hspace{-0.6 pt}\strikethroughcommand{#2}}_{\hspace{-0.6 pt}\vartriangle}}


%
% N A R R O W   P R O O F S   M A Y   B E   S P A C I O U S 
%-----------------------------------------------------------
%

%
% PEBBLING FORMULAS
%

\newcommand{\pebtreecontr}[2][h]{\pebcontr[{T_{#1}}]{#2}}
\newcommand{\pebtreecontrNT}[2][]{\pebcontrNT[T_{#1}]{#2}}
\newcommand{\pebsubtreecontrNT}[2]{\pebcontrNT[\binsubtree{#1}]{#2}}


%
% S-PEBBLING TERMINOLOGY
%

\newcommand{\spebblingtext}{\mbox{S-peb}\-bling\xspace}
\newcommand{\spebblinggame}{\mbox{S-peb}\-ble game\xspace}
\newcommand{\spebbling}[1][S]{\pebbling[#1]}
\newcommand{\sconf}[1][S]{\pconf[#1]}
\newcommand{\spebblingprice}[1]{\formatpebblingprice{S-Peb}(#1)}

%
% LABELLED PEBBLING (L-PEBBLING) TERMINOLOGY
%

\newcommand{\revwasteful}{wasteful\xspace}
\newcommand{\Revwasteful}{Wasteful\xspace}
\newcommand{\revnonwasteful}{non-wasteful\xspace}
\newcommand{\Revnonwasteful}{Non-wasteful\xspace}

\newcommand{\lctext}{\mbox{L-con}\-figu\-ra\-tion\xspace}
\newcommand{\lpebblingtext}{\mbox{L-peb}\-bling\xspace}
\newcommand{\lpebblingtextfull}{labelled pebbling\xspace}
\newcommand{\LPEBBLINGTEXT}{\mbox{L-peb}\-bling\xspace}
\newcommand{\lpebblinggame}{\mbox{L-peb}\-ble game\xspace}
\newcommand{\lpebblegame}{\mbox{L-peb}\-ble game\xspace}
\newcommand{\lpebblegamefull}{labelled pebble game\xspace}
\newcommand{\Lpebblegamefull}{Labelled pebble game\xspace}
\newcommand{\LPEBBLEGAMEFULL}{Labelled Pebble Game\xspace}
\newcommand{\lpebble}{\mbox{L-peb}\-ble\xspace}
\newcommand{\LPEBBLE}{\mbox{L-peb}\-ble\xspace}
\newcommand{\lpebblefull}{labelled pebble\xspace}

\newcommand{\Subconftext}{Sub\-con\-figu\-ration\xspace}
\newcommand{\subconftext}{sub\-con\-figu\-ration\xspace}

\newcommand{\lnonover}{non-over\-lapping\xspace}
\newcommand{\LNONOVER}{Non-Over\-lapping\xspace}
\newcommand{\lover}{over\-lapping\xspace}
\newcommand{\lnontouching}{non-touching\xspace}
\newcommand{\ltouching}{touching\xspace}

% OBSOLETE---REPLACE
\newcommand{\blunconditional}{independent\xspace}
\newcommand{\blconditional}{dependent\xspace}
\newcommand{\blconditionedon}{dependent on\xspace}
% WITH THIS:
\newcommand{\blindependent}{independent\xspace}
\newcommand{\bldependent}{dependent\xspace}
\newcommand{\bldependenton}{dependent on\xspace}

\newcommand{\ppos}{purely positive\xspace}
\newcommand{\pneg}{purely negative\xspace}

%
% LABELLED PEBBLING (L-PEBBLING) NOTATION
%

\newcommand{\lpebbling}[1][L]{\pebbling[#1]}
\newcommand{\lconf}[1][L]{\pconf[#1]}

\newcommand{\mconf}[1][M]{\pconf[#1]}

\newcommand{\lcost}[1]{\formatpebblingprice{cost}( #1 )}
\newcommand{\lcostcompact}[1]{\formatpebblingprice{cost}\bigl( #1 \bigr)}

\newcommand{\lpebblingprice}[1]{\formatpebblingprice{L-Peb}(#1)}
\newcommand{\lpebblingpricecompact}[1]% 
    {\formatpebblingprice{L-Peb}\bigl(#1\bigr)}

% Subconfigurations
\newcommand{\scnot}[2]{#1 \langle #2 \rangle}
\newcommand{\scnotcompact}[2]{#1 \bigl\langle #2 \bigr\rangle}

\newcommand{\scnotstd}{\scnot{v}{W}}

% Special subconfigurations
\newcommand{\introsubconfnot}[1]{\scnot{#1}{\prednode{#1}}}
\newcommand{\introsubconfnotcompact}[1]{\scnotcompact{#1}{\prednode{#1}}}
\newcommand{\unconditionalblacknot}[1]{\scnot{#1}{\emptyset}}

% Order relation on subconfigurations
\newcommand{\spleq}{\preceq}
\newcommand{\spgeq}{\succeq}
\newcommand{\spnotleq}{\not\preceq}
\newcommand{\spnotgeq}{\not\succeq}
\newcommand{\splt}{\prec}
\newcommand{\spgt}{\succ}
\newcommand{\spequal}{\sim}

% Subconfiguration merger
\newcommand{\spmerge}[2]
        {\formatfunctiontosubconfiguration{merge}(#1, #2 )}
\newcommand{\spmergecompact}[2]
        {\formatfunctiontosubconfiguration{merge}\bigl({#1}, {#2}\bigr)}

% Canonic subconfiguration representation
\newcommand{\spcanonconf}[1]{\formatfunctiontosubconfiguration{canon}({#1})}
\newcommand{\spcanonconfcompact}[1]%
        {\formatfunctiontosubconfiguration{canon}\bigl({#1}\bigr)}

% Subconfiguration projection
\newcommand{\spprojsubsub}[4]%
    {\formatfunctiontosubconfiguration{proj}_{\scnot{#1}{#2}}(\scnot{#3}{#4})}
\newcommand{\spprojsubsubcompact}[4]%
    {\formatfunctiontosubconfiguration{proj}_{\scnot{#1}{#2}}%
    \bigl(\scnot{#3}{#4}\bigr)}
\newcommand{\spprojsubconf}[3]%
    {\formatfunctiontosubconfiguration{proj}_{\scnot{#1}{#2}}({#3})}
\newcommand{\spprojsubconfcompact}[3]%
    {\formatfunctiontosubconfiguration{proj}_{\scnot{#1}{#2}}\bigl({#3}\bigr)}
\newcommand{\spprojconfsub}[3]%
    {\formatfunctiontosubconfiguration{proj}_{#1}(\scnot{#2}{#3})}
\newcommand{\spprojconfsubcompact}[3]%
    {\formatfunctiontosubconfiguration{proj}_{#1}\bigl(\scnot{#2}{#3}\bigr)}
\newcommand{\spprojconfconf}[2]%
    {\formatfunctiontosubconfiguration{proj}_{#1}({#2})}
\newcommand{\spprojconfconfcompact}[2]%
    {\formatfunctiontosubconfiguration{proj}_{#1}\bigl({#2}\bigr)}

% Functions from subconfigurations to sets of vertices 
% (closure, cover, internal, boundary)
\newcommand{\spclostext}{closure\xspace}
\newcommand{\spclossub}[2]{\formatfunctiontoset{cl}(\scnot{#1}{#2})}
\newcommand{\spclossubcompact}[2]%
        {\formatfunctiontoset{cl}\bigl(\scnotcompact{#1}{#2}\bigr)}
\newcommand{\spclosconf}[1]{\formatfunctiontoset{cl}({#1})}
\newcommand{\spclosconfcompact}[1]{\formatfunctiontoset{cl}\bigl({#1}\bigr)}

\newcommand{\spintersub}[2]{\formatfunctiontoset{int}(\scnot{#1}{#2})}
\newcommand{\spintersubcompact}[2]%
        {\formatfunctiontoset{int}\bigl(\scnotcompact{#1}{#2}\bigr)}
\newcommand{\spinterconf}[1]{\formatfunctiontoset{int}({#1})}
\newcommand{\spinterconfcompact}[1]{\formatfunctiontoset{int}\bigl({#1}\bigr)}

\newcommand{\spcoversub}[2]{\formatfunctiontoset{cover}(\scnot{#1}{#2})}
\newcommand{\spcoversubcompact}[2]%
        {\formatfunctiontoset{cover}\bigl(\scnotcompact{#1}{#2}\bigr)}
\newcommand{\spcoverconf}[1]{\formatfunctiontoset{cover}({#1})}
\newcommand{\spcoverconfcompact}[1]%
        {\formatfunctiontoset{cover}\bigl({#1}\bigr)}
\newcommand{\spboundarysub}[2]{\partial\scnot{#1}{#2}}
\newcommand{\spboundaryconf}[1]{\partial{#1}}

% Black and white pebbles in L-configuration
\newcommand{\spinducedblack}[1]%
    {\formatfunctiontoset{Bl} (#1)}
\newcommand{\spinducedwhite}[1]%
    {\formatfunctiontoset{Wh} (#1)}
\newcommand{\spinducedblackcompact}[1]%
    {\formatfunctiontoset{Bl} \bigl(#1 \bigr)}
\newcommand{\spinducedwhitecompact}[1]%
    {\formatfunctiontoset{Wh} \bigl(#1 \bigr)}


%
% INTERPRETATION OF CLAUSE SETS IN TERMS OF PEBBLES
%

% Induced L-configuration
\newcommand{\linducedconf}[1]{\lconf(#1)}

% Supporting white pebbles 
\newcommand{\wsuppspec}[2]{\formatfunctiontoset{swp} ( #1, #2 )}

% Witness clauses
\newcommand{\pathclause}[1]{\somenodetrueclause{\vertexpath{#1}}}
\newcommand{\pathclauseNR}[1]{\somenodetrueclause{\vertexpathNR{#1}}}
\newcommand{\pathclausedeg}[2][\pebdeg]%
    {\somenodetrueclausedeg[#1]{\vertexpath{#2}}}
\newcommand{\pathclauseNRdeg}[2][\pebdeg]%
    {\somenodetrueclausedeg[#1]{\vertexpathNR{#2}}}

\newcommand{\pathclausekplusone}[1]{\pathclausedeg[\clwidth+1]{#1}}
\newcommand{\pathclauseNRkplusone}[1]{\pathclauseNRdeg[\clwidth+1]{#1}}


% Support
\newcommand{\blacktruth}[1]{\clausesetformat{B} ( {#1} )}
\newcommand{\blacktruthcompact}[1]{\clausesetformat{B} \bigl( {#1} \bigr)}
\newcommand{\blacktruthsmall}[1]{\clausesetformat{B} ( {#1} )}

\newcommand{\blacktruthdeg}[2][d]{\clausesetformat{B}^{#1} ( {#2} )}
\newcommand{\blacktruthdegcompact}[2][d]{\clausesetformat{B}^{#1} \bigl( {#2} \bigr)}
\newcommand{\blacktruthdegsmall}[2][d]{\clausesetformat{B}^{#1} ( {#2} )}

\newcommand{\blacktruthkplusone}[1]{\blacktruthdeg[\clwidth + 1]{#1}}
\newcommand{\blacktruthkplusonecompact}[1]{\blacktruthdegcompact[\clwidth + 1]{#1}}
\newcommand{\blacktruthkplusonesmall}[1]{\blacktruthdegsmall[\clwidth + 1]{#1}}


% vertex, index, pegdegree, vertex set 
\newcommand{\blacktruthdegexplicit}[4]% 
        {\setdescrcompact
        {{\textstyle \Lor_{#2 = 1}^{#3} {#1}_{#2}}}
        {{#1} \in {#4}}}


%
% VERTICES AND VERTEX SETS
%

\newcommand{\binsubtree}[1]{T^{#1}}
\newcommand{\binsubtreeNR}[1]{T_{*}^{#1}}

\newcommand{\vertexpath}[1]{{P}^{#1}}
\newcommand{\vertexpathNR}[1]{{P}_{*}^{#1}}

\newcommand{\unrelatedNP}[1]%
        {T \setminus \bigl(\binsubtree{#1} \unionSP \vertexpath{#1} \bigr)}
\newcommand{\unrelatedsmallNP}[1]%
        {T \setminus (\binsubtree{#1} \unionSP \vertexpath{#1} )}
\newcommand{\unrelated}[1]{\bigl( \unrelatedNP{#1} \bigr)}

\newcommand{\complvertexpath}[1]{T \setminus \vertexpath{#1}}
\newcommand{\complvertexpathNR}[1]{T \setminus \vertexpathNR{#1}}

\newcommand{\complbinsubtree}[1]{T \setminus \binsubtree{#1}}
\newcommand{\complbinsubtreeNR}[1]{T \setminus \binsubtreeNR{#1}}


%
% K L A W E   P Y R A M I D   P E B B L I N G   L O W E R   B O U N D 
%---------------------------------------------------------------------
%

%    
% LAYERED GRAPHS   
%    

% Vertex levels
\DeclareMathOperator{\levelop}{level}
\DeclareMathOperator{\minlevelop}{minlevel}
\DeclareMathOperator{\maxlevelop}{maxlevel}

\newcommand{\vlevel}[1]{\levelop({#1})}
\newcommand{\vminlevel}[1]{\minlevelop({#1})}
\newcommand{\vmaxlevel}[1]{\maxlevelop({#1})}
\newcommand{\vlevelcompact}[1]{\levelop \bigl( {#1} \bigr)}
\newcommand{\vminlevelcompact}[1]{\minlevelop \bigl( {#1} \bigr)}
\newcommand{\vmaxlevelcompact}[1]{\maxlevelop \bigl( {#1} \bigr)}

\newcommand{\levelstd}{L}
\newcommand{\levelmin}{\levelstd}
%    \newcommand{\levelmin}{L_{\mathrm{min}}}
\newcommand{\levelmax}{L_{U}}
%    \newcommand{\levelmax}{L_{\mathrm{max}}}

% Topological sorting of vertices
\DeclareMathOperator{\topvertexop}{top}
\DeclareMathOperator{\bottomvertexop}{bot}

\newcommand{\maxvertex}[1]{\topvertexop(#1)}
\newcommand{\topvertex}[1]{\topvertexop(#1)}

\newcommand{\minvertex}[1]{\bottomvertexop(#1)}
\newcommand{\bottomvertex}[1]{\bottomvertexop(#1)}
  
\newcommand{\maxelement}[1]{{#1}_{\top}}
% Use just b instead of b_\bot
%    \newcommand{\minelement}[1]{{#1}_{\bot}}
\newcommand{\minelement}[1]{#1}

\newcommand{\maxelementtext}{top element\xspace}
\newcommand{\minelementtext}{bottom element\xspace}

\newcommand{\topvertices}[1]{\topvertexop(#1)}
%    \newcommand{\topvertices}[1]{\formatfunctiontoset{top} ( #1 )}
\newcommand{\topvertexadj}{top\xspace}
\newcommand{\topverticestext}{\topvertexadj vertices\xspace}
\newcommand{\topvertextext}{\topvertexadj vertex\xspace}

%
% PYRAMID GRAPHS
%
    
% Optional argument is height
%
% Something seems to be broken with this macro. It composes badly with
% other macros (see e.g. def of \pebpyramidcontr) and does not work
% in subfigure captions. Don't know why.
%
\newcommand{\pyramidgraph}[1][]{\Pi_{#1}}
\newcommand{\pyramidgraphh}{\pyramidgraph[h]}

\newcommand{\aboveverticespyramid}[1]{\abovevertices[\pyramidgraph]{#1}}
\newcommand{\aboveverticespyramidNR}[1]{\aboveverticesNR[\pyramidgraph]{#1}}
\newcommand{\belowverticespyramid}[1]{\belowvertices[\pyramidgraph]{#1}}
\newcommand{\belowverticespyramidNR}[1]{\belowverticesNR[\pyramidgraph]{#1}}

%
% PEBBLING CONTRADICTIONS OVER PYRAMIDS
%

\newcommand{\pebpyramidcontrNT}[2][]{\pebcontrNT[\Pi_{#1}]{#2}}
\newcommand{\pebpyramidcontr}[2][]{\pebcontr[\Pi_{#1}]{#2}}

%
% NOTATION AND TERMINOLOGY FOR PATHS
%

%    \newcommand{\sourcepath}{sourcepath\xspace}
\newcommand{\sourcepath}{source path\xspace}
\newcommand{\sinkpath}{sink path\xspace}
\newcommand{\sourcesinkpath}{source-sink path\xspace}
\newcommand{\Sourcepath}{Source path\xspace}
\newcommand{\Sinkpath}{Sink path\xspace}
\newcommand{\Sourcesinkpath}{Source-sink path\xspace}

\newcommand{\pathsoperator}{\mathfrak{P}}
%    \newcommand{\pathsoperator}{\formatfunctiontoset{paths}}
%    \DeclareMathOperator{\pathsoperator}{paths}
%    \newcommand{\setofpathsstd}{\mathcal{P}}    
\newcommand{\setofpathsstd}{\mathfrak{P}}
%    \newcommand{\setofpathsstd}{\mathcal{Q}}

\newcommand{\pathsop}{\pathsoperator_{\textrm{via}}}
\newcommand{\pathsviaop}{\pathsoperator_{\textrm{via}}}
\newcommand{\pathsinop}{\pathsoperator_{\textrm{in}}}
%    \newcommand{\pathsinop}{\mathcal{P}_{\textrm{in}}}
%    \newcommand{\pathsop}{\mathcal{P}_{\textrm{via}}}
%    \newcommand{\pathsviaop}{\mathcal{P}_{\textrm{via}}}

\newcommand{\pathsviavertex}[1]{\pathsviaop(#1)}
\newcommand{\pathsviavertexcompact}[1]{\pathsviaop \bigl ( #1 \bigr ) }
\newcommand{\pathsinvertex}[1]{\pathsinop(#1)}
\newcommand{\pathsinvertexcompact}[1]{\pathsinop \bigl ( #1 \bigr ) }
%
\newcommand{\unionpathsviavertex}[1]{\Union \pathsviaop(#1)}
\newcommand{\unionpathsviavertexcompact}[1]{\Union \pathsviaop \bigl ( #1 \bigr ) }
\newcommand{\unionpathsinvertex}[1]{\Union \pathsinop(#1)}
\newcommand{\unionpathsinvertexcompact}[1]{\Union \pathsinop \bigl ( #1 \bigr ) }

% Obsolete things below
\newcommand{\pathsvertex}[1]{\pathsinvertex{#1}}
\newcommand{\pathsviachain}[1]{\pathsviavertex{#1}}
\newcommand{\pathsviachaincompact}[1]{\pathsviavertexcompact{#1}}

%
% HIDING SET TERMINOLOGY AND NOTATION
%

\newcommand{\tightnessklawe}{tightness\xspace}
\newcommand{\tightklawe}{tight\xspace}
\newcommand{\Tightklawe}{Tight\xspace}
\newcommand{\connectedklawe}{\hidingklawe-connected\xspace}
\newcommand{\connectednessklawe}{\hidingklawe-connectedness\xspace}
\newcommand{\hideklawe}{hide\xspace}
\newcommand{\Hideklawe}{Hide\xspace}
\newcommand{\hiddenklawe}{hidden\xspace}
\newcommand{\Hiddenklawe}{Hidden\xspace}
\newcommand{\hidingklawe}{hiding\xspace}
\newcommand{\Hidingklawe}{Hiding\xspace}
\newcommand{\hidingsetklawe}{hiding set\xspace}
\newcommand{\Hidingsetklawe}{Hiding set\xspace}            
\newcommand{\necessaryhidingsetklawe}{necessary hiding subset\xspace}
\newcommand{\Necessaryhidingsetklawe}{Necessary hiding subset\xspace}

\newcommand{\hidsetgraph}{\mathcal{H}}

%
% VERTEX SET MEASURE AND POTENTIAL
%

\newcommand{\minmeasure}{minimum-measure\xspace}
\newcommand{\minsize}{minimum-size\xspace}
\newcommand{\subsetminimal}{subset-minimal\xspace}
\newcommand{\Minmeasure}{Minimum-measure\xspace}
\newcommand{\Minsize}{Minimum-size\xspace}
\newcommand{\Subsetminimal}{Subset-minimal\xspace}

\DeclareMathOperator{\blsegmentop}{seg}              % OBSOLETE?
\newcommand{\blsegment}[2]{\blsegmentop_{#1}({#2})}  % OBSOLETE?
\newcommand{\dummybottomvertex}{\bot}                % OBSOLETE?

\DeclareMathOperator{\potentialop}{pot}

\newcommand{\vpotential}[2][]{\potentialop_{#1}({#2})}

\newcommand{\meastopot}[2][]{\vmeasure[#1]{#2}}

%
% BLACK-WHITE PEBBLING LOWER BOUND ASSUMING KLAWE PROPERTY / LHC PROPERTY
%

\newcommand{\vertabovelevel}[2]{{#1} \{ {\succeq\!#2} \} }
\newcommand{\vertstrictlyabovelevel}[2]{{#1} \{ {\succ\!#2} \} }
\newcommand{\vertbelowlevel}[2]{{#1} \{ {\preceq\!#2} \} }
\newcommand{\vertstrictlybelowlevel}[2]{{#1} \{ {\prec\!#2} \} }
\newcommand{\vertonlevel}[2]{{#1} \{ {\sim\!#2} \} }

\newcommand{\abovelevelblockerminsize}[2]{L_{\succeq{#1}}({#2})}
\newcommand{\abovelevelblockerminsizecompact}%
    [2]{L_{\succeq{#1}}\bigl({#2}\bigr)}

\newcommand{\vjthmeasure}[3][]{m_{#1}^{#2} ( {#3} ) }
\newcommand{\vmeasure}[2][]{m_{#1} ( {#2} ) }
\newcommand{\Vjthmeasure}[3][]{m_{#1}^{#2} \bigl( {#3} \bigr) }
\newcommand{\Vmeasure}[2][]{m_{#1} \bigl( {#2} \bigr) }

%OBSOLETE
\newcommand{\vjthmeasurecompact}[3][]{m_{#1}^{#2} \bigl( {#3} \bigr) }
\newcommand{\vmeasurecompact}[2][]{m_{#1} \bigl( {#2} \bigr) }

\newcommand{\measureleq}{\precsim_{m}}

\newcommand{\hiddenvertices}[1]{\llceil {#1} \rrceil}
%\newcommand{\hiddenverticescompact}[1]{\bigl \llceil {#1} \bigr \rrceil}
% Seems that delimiters \llceil and \rrceil do not work together with
% \bigl and \bigr ?!

\newcommand{\necessaryhidingvert}[2]%
{{#1}{\scriptstyle{\llfloor {#2} \rrfloor}}}
%\newcommand{\necessaryhidingvert}[2]%
%    {{#1}{\scriptscriptstyle{\llfloor {#2} \rrfloor}}}


%
% KLAWE PROPERTY / LHC PROPERTY TERMINOLOGY
%

\newcommand{\klawepropertyprefix}{limited hiding-cardinality\xspace}
\newcommand{\Klawepropertyprefix}{Limited hiding-cardinality\xspace}
\newcommand{\KLAWEPROPERTYPREFIX}{Limited Hiding-Cardinality\xspace}

\newcommand{\klawepropacronym}{LHC property\xspace}
\newcommand{\localklawepropacronym}{Local LHC property\xspace}
\newcommand{\genklawepropacronym}{Generalized LHC property\xspace}
\newcommand{\GENKLAWEPROPACRONYM}{Generalized LHC Property\xspace}

\newcommand{\klaweprop}{\Klawepropertyprefix property\xspace}
\newcommand{\Klaweprop}{\Klawepropertyprefix property\xspace}
\newcommand{\KLAWEPROP}{\KLAWEPROPERTYPREFIX Property\xspace}

\newcommand{\localklaweprop}{Local \klawepropertyprefix property\xspace}
\newcommand{\Localklaweprop}{Local \klawepropertyprefix property\xspace}
\newcommand{\LOCALKLAWEPROP}{Local \KLAWEPROPERTYPREFIX property\xspace}

\newcommand{\genklaweprop}{Generalized \klawepropertyprefix property\xspace}
\newcommand{\Genklaweprop}{Generalized \klawepropertyprefix property\xspace}
\newcommand{\GENKLAWEPROP}{Generalized \KLAWEPROPERTYPREFIX Property\xspace}

\newcommand{\nongenklaweprop}%
{non-generalized \Klawepropertyprefix property\xspace}
\newcommand{\nongenklawepropacronym}%
{non-generalized \klawepropacronym}
\newcommand{\nongenklawepropacronymWithParam}%
{(non-generalized) \klawepropacronym}

\newcommand{\gkpconstant}{C_{K}}


%
% PROOF OF SPREADING PROPERTY: NOTATION AND TERMINOLOGY 
%

\newcommand{\nepath}{\mbox{NE-path}\xspace}        
\newcommand{\nepathlong}{north-east path\xspace}        
\newcommand{\nwpath}{\mbox{NW-path}\xspace}        
\newcommand{\nwpathlong}{north-west path\xspace}        

\newcommand{\nepaththrough}[1]{P_{\textrm{NE}}({#1})}
\newcommand{\nwpaththrough}[1]{P_{\textrm{NW}}({#1})}


%    
% T O W A R D S   O P T I M A L   S E P A R A T I O N   
%-----------------------------------------------------    
%    

%
% RESTRICTION ON GRAPHS
%

\newcommand{\siblingnonreachabiblitypropertynoref}%
{Sibling non-reachability property\xspace}
\newcommand{\Siblingnonreachabiblitypropertynoref}%
{Sibling non-reachability property\xspace}
\newcommand{\siblingnonreachabiblityproperty}%
{\siblingnonreachabiblitypropertynoref~% 
\ref{property:sibling-non-reachability-property}\xspace}
\newcommand{\Siblingnonreachabiblityproperty}%
{\Siblingnonreachabiblitypropertynoref~%
\ref{property:sibling-non-reachability-property}\xspace}

%    \newcommand{\pebblingdag}{\multipebblingtext DAG\xspace}
%    \newcommand{\Pebblingdag}{\Multipebblingtext DAG\xspace}
\newcommand{\pebblingdag}{blob-pebblable DAG\xspace}
\newcommand{\Pebblingdag}{Blob-pebblable DAG\xspace}

\newcommand{\pebblingdagadj}{blob-pebblable\xspace}

%
% BLOB-PEBBLING TERMINOLOGY
%
% The macros refer to the old multipebbling terminology instead of 
% the new blob-pebbling terminology 
% 
% Abbreviations \mpsc-something usually denote subconfigurations.
% A subconfiguration is a black blob with supporting white pebbles
%
% Abbreviations \mpc-something usually denote blob-pebbling 
% configurations (that are sets of subconfigurations).
%

\newcommand{\mergervertextext}{merger vertex\xspace}
\newcommand{\mergervertex}{v^*}

\newcommand{\introducetermanmpctext}%
    {a \introduceterm{\mpctext{}}\xspace}

\newcommand{\introducetermamultipebblingtext}%
  {a \introduceterm{\multipebblingtext{}}\xspace}

\newcommand{\blobpebblingtext}{blob-pebbling\xspace}
\newcommand{\Blobpebblingtext}{Blob-pebbling\xspace}
\newcommand{\BLOBPEBBLINGTEXT}{Blob-Pebbling\xspace}

\newcommand{\amultipebblingtext}{a \blobpebblingtext}
\newcommand{\Amultipebblingtext}{A \blobpebblingtext}
\newcommand{\anmpebblingtext}{a \blobpebblingtext}
\newcommand{\Anmpebblingtext}{A \blobpebblingtext}
%    \newcommand{\amultipebblingtext}{a multi-pebbling\xspace}
%    \newcommand{\Amultipebblingtext}{A multi-pebbling\xspace}
%    \newcommand{\anmpebblingtext}{an M-pebbling\xspace}
%    \newcommand{\Anmpebblingtext}{An M-pebbling\xspace}

\newcommand{\mpebblingtext}{\blobpebblingtext}
\newcommand{\Mpebblingtext}{\Blobpebblingtext}
\newcommand{\MPEBBLINGTEXT}{\BLOBPEBBLINGTEXT}
%    \newcommand{\mpebblingtext}{M-pebbling\xspace}
%    \newcommand{\Mpebblingtext}{M-pebbling\xspace}
%    \newcommand{\MPEBBLINGTEXT}{M-Pebbling\xspace}

\newcommand{\multipebblingtext}{\blobpebblingtext}
\newcommand{\Multipebblingtext}{\Blobpebblingtext}
\newcommand{\MULTIPEBBLINGTEXT}{\BLOBPEBBLINGTEXT}

\newcommand{\blobpebblegame}{blob-pebble game\xspace}
\newcommand{\Blobpebblegame}{Blob-pebble game\xspace}
\newcommand{\BLOBPEBBLEGAME}{Blob-Pebble Game\xspace}
\newcommand{\multipebblegame}{blob-pebble game\xspace}
\newcommand{\Multipebblegame}{Blob-pebble game\xspace}
\newcommand{\MULTIPEBBLEGAME}{Blob-Pebble Game\xspace}
%    \newcommand{\multipebblegame}{multi-pebble game\xspace}
%    \newcommand{\Multipebblegame}{Multi-pebble game\xspace}
%    \newcommand{\MULTIPEBBLEGAME}{Multi-Pebble Game\xspace}

%    \newcommand{\multipebblenotblob}{multi-pebble\xspace}
%    \newcommand{\MULTIPEBBLENOTBLOB}{Multi-Pebble\xspace}
\newcommand{\multipebble}{blob\xspace}
\newcommand{\Multipebble}{Blob\xspace}
\newcommand{\MULTIPEBBLE}{Blob\xspace}

\newcommand{\blobpebble}{blob-pebble\xspace}
\newcommand{\Blobpebble}{Blob-pebble\xspace}
\newcommand{\BLOBPEBBLE}{Blob-Pebble\xspace}
\newcommand{\blob}{blob\xspace}
\newcommand{\Blob}{Blob\xspace}
\newcommand{\BLOB}{Blob\xspace}
%    \newcommand{\multipebble}{multi-pebble\xspace}
%    \newcommand{\Multipebble}{Multi-pebble\xspace}
%    \newcommand{\MULTIPEBBLE}{Multi-Pebble\xspace}

\newcommand{\multipebbleprefix}{blob-\xspace}
%    \newcommand{\multipebbleprefix}{multi-\xspace}
\newcommand{\atomicmultipebbleadj}{atomic\xspace}
\newcommand{\Atomicmultipebbleadj}{Atomic\xspace}
\newcommand{\anatomicmultipebbleadj}{an \atomicmultipebbleadj}
\newcommand{\Anatomicmultipebbleadj}{An \atomicmultipebbleadj}

%
% BLOB-PEBBLING NOTATION
%

\newcommand{\blobpebbling}[1][P]{\pebbling[#1]}
\newcommand{\multipebbling}[1][P]{\pebbling[#1]}
\newcommand{\mpconf}[1][S]{\pconf[#1]}

\newcommand{\mpcost}[1]{\formatpebblingprice{cost}( #1 )}
\newcommand{\mpcostcompact}[1]{\formatpebblingprice{cost}\bigl( #1 \bigr)}

\newcommand{\mpcostblack}[1]%
        {\formatpebblingprice{cost}_{\mpcblacks}( #1 )}
\newcommand{\mpcostwhite}[1]%
        {\formatpebblingprice{cost}_{\mpcwhites}( #1 )}


\newcommand{\blobpebblingprice}[1]{\formatpebblingprice{Blob-Peb}(#1)}
\newcommand{\blobpebblingpricecompact}[1]% 
    {\formatpebblingprice{Blob-Peb}\bigl(#1\bigr)}
\newcommand{\multipebblingprice}[1]{\formatpebblingprice{Blob-Peb}(#1)}
\newcommand{\multipebblingpricecompact}[1]% 
    {\formatpebblingprice{Blob-Peb}\bigl(#1\bigr)}

%lpp stands for legal pebble positions
\newcommand{\lpptext}{legal pebble positions\xspace}
\newcommand{\lpptextsing}{legal pebble position\xspace}
\newcommand{\Lpptext}{Legal pebble positions\xspace}

\newcommand{\lpp}[1]{\formatfunctiontoset{lpp} ( #1 )}
\newcommand{\lppstd}{\lpp{B}}

%\lppdefinition{multi-pebble}{bottom element}
\newcommand{\lppdefinition}[2]{\belowverticesNR{#2} \unionSP
        (\unionpathsinvertex{#1} \setminus {#1})}

\newcommand{\lppdefinitionstd}{\lppdefinition{B}{b}}
%\newcommand{\lppdefinitionstd}{\lppdefinition{B}{\minelement{b}}}

\newcommand{\pathsBminusB}{\pathsvertex{B} \setminus{B}}


%
% BLOB-PEBBLING CONFIGURATIONS AND SUBCONFIGURATIONS
%

\newcommand{\mpcblacks}{\formatfunctiontomulti{B}}
\newcommand{\mpcwhites}{\formatfunctiontomulti{W}}

\newcommand{\mpcblacksof}[1]{\formatfunctiontomulti{B}({#1})}
\newcommand{\mpcwhitesof}[1]{\formatfunctiontomulti{W}({#1})}

\newcommand{\mpscblacknot}[1]{[ {#1} ]}
\newcommand{\blackblobnot}[1]{\mpscblacknot{#1}}

\newcommand{\mpscnot}[2]{[ {#1} ] \langle {#2} \rangle}
\newcommand{\mpscnotcompact}[2]%
        {\big[ {#1} \big] \bigl\langle {#2} \bigr\rangle}

\newcommand{\mpscnotstd}[1][]{\mpscnot{B_{#1}}{W_{#1}}}
\newcommand{\mpscnotprime}{\mpscnot{B'}{W'}}
\newcommand{\mpscnotstar}{\mpscnot{B^{*}}{W^{*}}}

\newcommand{\bprime}{B'}
\newcommand{\wprime}{W'}
\newcommand{\bstar}{B^{*}}
\newcommand{\wstar}{W^{*}}

% Special subconfigurations
\newcommand{\rpqmpscnot}{\mpscnot{r}{p,q}}
\newcommand{\intrompscnot}[1]{\mpscnot{#1}{\prednode{#1}}}
\newcommand{\intrompscnotcompact}[1]{\mpscnotcompact{#1}{\prednode{#1}}}
\newcommand{\unconditionalblackmpscnot}[1]{\mpscnot{#1}{\emptyset}}

\newcommand{\Mpctext}{\Blobpebblingtext con\-fig\-u\-ra\-tion\xspace}
\newcommand{\mpctext}{\blobpebblingtext con\-fig\-u\-ra\-tion\xspace}
\newcommand{\MPCTEXT}{\BLOBPEBBLINGTEXT Con\-fig\-u\-ra\-tion\xspace}
\newcommand{\anmpctext}{a \mpctext}
\newcommand{\Anmpctext}{A \mpctext}
%    \newcommand{\mpctext}{\mbox{M-con}\-fig\-u\-ra\-tion\xspace}
%    \newcommand{\anmpctext}{an \mpctext}
%    \newcommand{\Anmpctext}{An \mpctext}

\newcommand{\Mpsctext}{Sub\-con\-figu\-ration\xspace}
\newcommand{\mpsctext}{sub\-con\-figu\-ration\xspace}
\newcommand{\Anmpsctext}{A sub\-con\-figu\-ration\xspace}
\newcommand{\anmpsctext}{a sub\-con\-figu\-ration\xspace}

\newcommand{\Mpscfulltext}{Blob sub\-con\-figu\-ration\xspace}
\newcommand{\mpscfulltext}{blob sub\-con\-figu\-ration\xspace}
\newcommand{\Anmpscfulltext}{A blob sub\-con\-figu\-ration\xspace}
\newcommand{\anmpscfulltext}{a blob sub\-con\-figu\-ration\xspace}
%\newcommand{\Mpscfulltext}{Multi-pebble sub\-con\-figu\-ration\xspace}
%\newcommand{\mpscfulltext}{multi-pebble sub\-con\-figu\-ration\xspace}

\newcommand{\predrequalpq}{\prednode{r} = \pqset}
\newcommand{\mpscrpq}{\mpscnot{r}{p,q}}


%
% INDUCED BLOB-PEBBLING CONFIGURATIONS
%

\newcommand{\mpinducedconf}[1]{\mpconf(#1)}

\newcommand{\mpinducedctminusone}{\mpinducedconf{\clsc_{t-1}}}
\newcommand{\mpinducedct}{\mpinducedconf{\clsc_{t}}}

% Precise / sharp implication
\newcommand{\preciseimpl}{\vartriangleright}
\newcommand{\notpreciseimpl}{\ntriangleright}
\newcommand{\sharpimpl}{\vartriangleright}
\newcommand{\notsharpimpl}{\ntriangleright}
%    \newcommand{\sharpimpl}{\blacktriangleright}
%    \newcommand{\notsharpimpl}{\not \blacktriangleright}
%    \newcommand{\sharpimpl}{\Vvdash}
%    \newcommand{\sharpimpladv}{sharply\xspace}
%    \newcommand{\sharpimplsubst}{sharp implication\xspace}
%    \newcommand{\sharpimplsharpness}{sharpness\xspace}
\newcommand{\sharpimpladv}{precisely\xspace}
\newcommand{\sharpimpladj}{precise\xspace}
\newcommand{\sharpimplsubst}{precise implication\xspace}
\newcommand{\Sharpimplsubst}{Precise implication\xspace}
\newcommand{\sharpimplsharpness}{preciseness\xspace}
\newcommand{\sharpimplpair}{precise implication pair\xspace}

\newcommand{\preciseimpladv}{precisely\xspace}
\newcommand{\preciseimpladj}{precise\xspace}
\newcommand{\preciseimplsubst}{precise implication\xspace}
\newcommand{\Preciseimplsubst}{Precise implication\xspace}
\newcommand{\preciseimplpreciseness}{preciseness\xspace}
\newcommand{\preciseimplpair}{precise implication pair\xspace}

% Some frequent multi-pebble configuration sets
\newcommand{\BuW}{B \unionSP W}
\newcommand{\Bup}{B \unionSP \singset{p}}
\newcommand{\Buq}{B \unionSP \singset{q}}
\newcommand{\Bur}{B \unionSP \singset{r}}
\newcommand{\Buv}{B \unionSP \singset{v}}
\newcommand{\Sur}{S \unionSP \singset{r}}
\newcommand{\Wur}{W \unionSP \singset{r}}
\newcommand{\Wup}{W \unionSP \singset{p}}
\newcommand{\Wuq}{W \unionSP \singset{q}}
\newcommand{\Wpuq}{W_p \unionSP \singset{q}}
\newcommand{\Wqup}{W_q \unionSP \singset{p}}
\newcommand{\WpuWq}{W_p \unionSP W_q}
\newcommand{\vrset}{\setsmall{v,r}}
\newcommand{\vrsetNP}{v,r}
\newcommand{\pqset}{\setsmall{p,q}}


%
% LARGE PEBBLING COST ==> MANY CLAUSES
%

\newcommand{\chargeabletext}{chargeable\xspace}        
\newcommand{\chargeableverticestext}{chargeable vertices\xspace}        
\newcommand{\Chargeableverticestext}{Chargeable vertices\xspace}        

\newcommand{\chargeablevertices}[1]%        
{\formatfunctiontoset{chargeable}({#1}) }
\newcommand{\chargeableverticescompact}[1]%        
{\formatfunctiontoset{chargeable}\bigl({#1}\bigr) }

\newcommand{\costcover}{cost-cover\xspace}        
\newcommand{\costcovers}{cost-covers\xspace}        
\newcommand{\costcovered}{cost-covered\xspace}        
\newcommand{\costcovering}{cost-covering\xspace}        

\newcommand{\blackschargedfor}[1][]% 
    {\mpcblacks_{#1}}
\newcommand{\whiteschargedfor}[1][]% 
    {\mpcwhites_{#1}^{\hspace{-0.3 pt}\vartriangle}}

% Notation in cost of induced >= size of set proof
\newcommand{\reprset}{R}
\newcommand{\reprsetprimed}{R'}
\newcommand{\reprsetith}{R[i]}
\newcommand{\reprvertex}{r}

%
% BLOB-PEBBLING LOWER BOUND ASSUMING GENERALIZED LHC
%

\DeclareMathOperator{\unblockedop}{unblocked}
\newcommand{\unblocked}[1]{\unblockedop({#1})}



%
% NOTATION AND TERMINOLOGY IN GENERALIZED LHC PROPERTY PROOF
%

\DeclareMathOperator{\elimop}{elim}

\newcommand{\welim}[2]{\text{$\mpcwhites$-$\elimop$}({#1}, {#2})}
\newcommand{\weliminate}{\mbox{$\mpcwhites$-elim}\-i\-nate\xspace}
\newcommand{\weliminated}{\mbox{$\mpcwhites$-elim}\-i\-nated\xspace}
\newcommand{\welimination}{\mbox{$\mpcwhites$-elim}\-i\-nation\xspace}

\newcommand{\kmatchedindex}{m}

\newcommand{\weightklawe}[1]{w({#1})}
\newcommand{\weightklawecompact}[1]{w\bigl({#1}\bigr)}

\newcommand{\ujustblocking}{U_B}
\newcommand{\uhiding}{U_H}
\newcommand{\uhidingith}[1][i]{U_{H}^{#1}}
\newcommand{\utight}{U_T}
\newcommand{\utightith}{U_{T}^{i}}

\newcommand{\unewblockingset}{U^{*}}

\newcommand{\unewhidingith}[1][i]{U_{*}^{#1}}

\newcommand{\mpconfjustblocked}{\mpconf_B}
\newcommand{\mpconfhidden}{\mpconf_H}

\newcommand{\blacksjustblocked}{\mpcblacks_B}
\newcommand{\blackshidden}{\mpcblacks_H}
\newcommand{\blackshiddenith}{\mpcblacks_{H}^{i}}

% ``Standard'' black bottom vertices
\newcommand{\bbvstd}{\mpcblacks}

\newcommand{\whitesbelowjustblocked}%
    {\mpcwhites_{B}^{\hspace{-0.3 pt}\vartriangle}}
\newcommand{\whitesbelowhidden}%
    {\mpcwhites_{H}^{\hspace{-0.3 pt}\vartriangle}}
\newcommand{\whitesbelowhiddenith}{\mpcwhites_{H}^{i}}
\newcommand{\whitestight}%
    {\mpcwhites_{T}^{\hspace{-0.3 pt}\vartriangle}}
\newcommand{\whitestightith}{\mpcwhites_{T}^{i}}


%    
% N O N - C H A I N   B L O B   P E B B L I N G   G A M E    
%---------------------------------------------------------    
%    

\newcommand{\canonminimsubst}{canonical minimization\xspace}
\newcommand{\Canonminimsubst}{Canonical minimization\xspace}

%
% LOWER BOUND COST OF INDUCED WHITE PEBBLES ==> CLAUSE SET SIZE
%

\newcommand{\wthin}{\mbox{$W$\!-thin}\xspace}
\newcommand{\wfat}{\mbox{$W$\!-fat}\xspace}


%    
% BLACK MULTIPEBBLES, COST OF BLACK MULTIPEBBLES ETC
%    

\newcommand{\uniquerepresentatives}{distinguished representatives\xspace}
\newcommand{\Uniquerepresentatives}{Distinguished representatives\xspace}
\newcommand{\soursing}{set of \uniquerepresentatives}
\newcommand{\sourplur}{sets of \uniquerepresentatives}
\newcommand{\psoursing}{partial \soursing}
\newcommand{\psourplur}{partial \sourplur}


%    
% S H O R T   P R O O F S   /   U N D E R S T A N D I N G   S P A C E 
%---------------------------------------------------------------------
%    

%
% !!! Things from tentativenotation-file should be inserted here !!!
%




==> notationProofComplexity.tex <==
%
%  N O T A T I O N   F O R   P R O O F   C O M P L E X I T Y   S T U F F
%------------------------------------------------------------------------
%
% AUTHOR
%
% Jakob Nordström <jakobn@kth.se>
%
% VERSION
%
% Last updated November 26, 2008
%    

%
% M I S C E L L A N E O U S 
%---------------------------
%

% Dots in x_1 \lor ... \lor x_n and the like
\newcommand{\formuladots}{\cdots}

% Implication and non-implication
\newcommand{\impl}{\vDash}
\newcommand{\nimpl}{\nvDash}

% Notation for singleton sets (To postpone decision with or without brackets?)
\newcommand{\singset}[1]{#1}

% Boundary
\newcommand{\boundary}[1]{\ensuremath{\partial #1}}

% Matching space(?)
\newcommand{\matchingspaceof}[1]{\genericform{MatchSp}{#1}}

%
% Used in Ben-Sasson and Wigderson: Short Proofs TO BE REMOVED?
%
%    \newcommand{\setofunsat}{{\ensuremath{\mathcal{A}}}}
%    \newcommand{\cplx}{{\ensuremath{\mu}}}
%    \newcommand{\cplxof}[2][\setofunsat]
%            {{\ensuremath{\cplx_{#1} (#2 )}}}
%    \newcommand{\cplxstd}{{\cplxof{\clc}}}


%
% S O M E   C O M M O N   T E R M S   A N D   E X P R E S S I O N S
%-------------------------------------------------------------------
%

\newcommand{\proplog}{propo\-sitional logic\xspace}
\newcommand{\tva}{truth value assignment\xspace}
\newcommand{\Tva}{Truth value assignment\xspace}

\newcommand{\fs}{Frege system\xspace}      % OBSOLETE?
\newcommand{\bdfs}{bounded depth \fs}      % OBSOLETE?

\newcommand{\psyst}{proof system\xspace}
\newcommand{\Psyst}{Proof system\xspace}
\newcommand{\PSYST}{Proof System\xspace}
\newcommand{\pps}{propo\-sitional proof system\xspace}
\newcommand{\Pps}{Propo\-sitional proof system\xspace}
\newcommand{\PPS}{Propo\-sitional Proof System\xspace}

\newcommand{\pproc}{proof procedure\xspace}
\newcommand{\Pproc}{Proof procedure\xspace}

\newcommand{\pmeth}{proof method\xspace}
\newcommand{\Pmeth}{Proof method\xspace}
\newcommand{\PMeth}{Proof Method\xspace}

\newcommand{\psa}{proof search algorithm\xspace}
\newcommand{\Psa}{Proof search algorithm\xspace}
\newcommand{\PSA}{Proof Search Algorithm\xspace}

\newcommand{\aut}{automatizable\xspace} 
\newcommand{\Aut}{Automatizable\xspace} 
\newcommand{\quasiaut}{quasi-\aut}
\newcommand{\autS}{automatizability\xspace} 
\newcommand{\AutS}{Automatizability\xspace} 

\newcommand{\psim}{\mbox{\ensuremath{p}-simu}\-lation\xspace}
\newcommand{\psiminf}{\mbox{\ensuremath{p}-simu}\-late\xspace}
\newcommand{\pbounded}{\mbox{\ensuremath{p}-bounded}\xspace}
\newcommand{\pequiv}{\mbox{\ensuremath{p}-equiv}\-a\-lent\xspace}
\newcommand{\pequivS}{\mbox{\ensuremath{p}-equiv}\-a\-lence\xspace}

\newcommand{\poptimal}{\mbox{\ensuremath{p}-optimal}\xspace}


%
% N O T A T I O N   F O R   P R O O F   S Y S T E M S 
%-----------------------------------------------------
%

\newcommand{\proofsystemformat}[1]{\ensuremath{\mathfrak{#1}}}

\newcommand{\prsyststd}{\proofsystemformat{P}}
\newcommand{\psstd}{\prsyststd}

\newcommand{\pprocstd}[1]{\ensuremath{A}_{#1}}

%    \newcommand{\pscompl}[1]{\mathit{comp}_{#1}}
\newcommand{\pscompl}[1]{\mathit{cplx}({#1})}

% Standard denotation of an arbitrary proof or derivation
\newcommand{\proofstd}{\ensuremath{\pi}}

% General notation for derivation rules
\newcommand{\derivrule}[2]{\frac{#1}{#2}}
\newcommand{\derivrulebinary}[3]{\frac{#1 \quad #2}{#3}}
\newcommand{\derivruleunary}[2]{\frac{#1}{#2}}
\newcommand{\derivruleaxiom}[1]{\frac{\ \ }{#1}}


%
% GENTZEN SEQUENT CALCULUS
%

\newcommand{\gentzensequent}[2]{\ensuremath{{#1} \vdash {#2}}}
\newcommand{\gentzensequentstd}
        {\gentzensequent{\fstd_1, \ldots, \fstd_n}{\fvar_1, \ldots, \fvar_m}}

\newcommand{\gentzenrule}[2]{\ensuremath{\frac{#1}{#2}}}
\newcommand{\gentzenbinrule}[3]{\gentzenrule{#1 \quad #2}{#3}}

\newcommand{\gentzenseqstd}{\ensuremath{\Gamma}}
\newcommand{\gentzenseqalt}{\ensuremath{\Delta}}

%
% FREGE SYSTEMS
%

% \bdfnot: bounded depth Frege
\newcommand{\bdfnot}[1][d]{\proofsystemformat{F}_{#1}}

%
% RESOLUTION AND FRIENDS
%

% \resnot: resolution
% \treeresnot: tree-like resolution
% \resknot: k-DNF resolution

\newcommand{\resnot}{\proofsystemformat{R}}
\newcommand{\treeresnot}{\proofsystemformat{T}}
%    \newcommand{\treeresnot}{\proofsystemformat{R}^*}

%    \newcommand{\resknot}[1][k]{\proofsystemformat{Res}({#1})}
\newcommand{\resknot}[1][k]{\proofsystemformat{R}({#1})}
\newcommand{\reskone}{\resknot[k+1]}



%
% R E S O L U T I O N  
%---------------------
%

%
% SOME TERMINOLOGY
%

\newcommand{\treelikeres}{tree-like resolution\xspace}
\newcommand{\Treelikeres}{Tree-like resolution\xspace}
\newcommand{\treeres}{tree resolution\xspace}
\newcommand{\Treeres}{Tree resolution\xspace}
\newcommand{\treeref}{tree-like refutation\xspace}
\newcommand{\treeresref}{\treelikeres refutation\xspace}

\newcommand{\resref}{resolution refutation\xspace}
\newcommand{\Resref}{Resolution refutation\xspace}
\newcommand{\RESREF}{Resolution Refutation\xspace}
\newcommand{\resderiv}{resolution derivation\xspace}
\newcommand{\Resderiv}{Resolution derivation\xspace}
\newcommand{\RESDERIV}{Resolution Derivation\xspace}
\newcommand{\resproof}{resolution proof\xspace}

\newcommand{\DPshort}{Davis-Putnam\xspace}
\newcommand{\DPproc}{\DPshort procedure\xspace}
\newcommand{\DPres}{\DPshort resolution\xspace}
\newcommand{\dpres}{\DPshort resolution\xspace}
\newcommand{\DPresshort}{\mbox{DP-reso}\-lu\-tion\xspace}
\newcommand{\dpresshort}{\mbox{DP-reso}\-lu\-tion\xspace}
\newcommand{\DLL}{DLL\xspace}
\newcommand{\dll}{DLL\xspace}
\newcommand{\dllproc}{DLL procedure\xspace}
\newcommand{\dllalg}{DLL algorithm\xspace}
\newcommand{\orderdll}{fixed-order DLL\xspace}

% Unit propagation or unit resolution
% purity checking or pure variable elimination
\newcommand{\unitprop}{unit propagation\xspace}
\newcommand{\unitpropalt}{unit resolution\xspace}
\newcommand{\purecheck}{purity checking\xspace}
\newcommand{\purecheckalt}{pure variable elimination\xspace}

% Trade-offs
\newcommand{\lwtradeoff}{length-width trade-off\xspace}
\newcommand{\lstradeoff}{length-space trade-off\xspace}
\newcommand{\wstradeoff}{width-space trade-off\xspace}

%
% RESOLUTION NOTATION
%

\newcommand{\resstd}{\ensuremath{\pi}}  % OBSOLETE---USE \proofstd INSTEAD

\newcommand{\derives}{\vdash}
\newcommand{\derivof}[4][\derives]
        {{\ensuremath{{#2} : {#3} \, {#1}\, {#4}}}}
%    \newcommand{\derivof}[3]{\ensuremath{#1 : #2 \vdash #3}}

\newcommand{\derivofall}[3]{\derivof[\deriveswithall]{#1}{#2}{#3}}

\newcommand{\refof}[2]{\derivof{#1}{#2}{\falsenum}}

\newcommand{\resderivspacesequence}[1]{\setsmall{#1}}


% Resolution derivation with all clauses used
\newcommand{\deriveswithall}%
        {\vdash_{\!\!\!{\scriptscriptstyle \forall}}} 
\newcommand{\notderiveswithall}%
        {\nvdash_{\!\!\!{\scriptscriptstyle \forall}}} 
%    \newcommand{\deriveswithall}{\vdash^{\!\!\forall}}
%    \newcommand{\deriveswithall}{\vdash_{\!\!\forall}}
%    \newcommand{\notderiveswithall}{\not \vdash^{\!\!\forall}}


% Format of resolution rule schemas or applications

\newcommand{\resrule}[3]{\derivrulebinary{#1}{#2}{#3}}
\newcommand{\thinrule}[2]{\derivruleunary{#1}{#2}}

%    OBSOLETE
%    \newcommand{\resrule}[3]{{\ensuremath{\frac{#1 \quad #2}{#3}}}}
%    \newcommand{\thinrule}[2]{{\ensuremath{\frac{#1}{#2}}}}

\newcommand{\resolventof}[2]{\ensuremath{\mathit{Res}({#1}, {#2})}}

% Transitions between clause configurations
\newcommand{\clcfgtransition}[2]{\ensuremath{#1 \rightsquigarrow #2}}
\newcommand{\clcfgtransitioncrammed}[2]%
        {\ensuremath{#1 \!\rightsquigarrow\! #2}}

%
% N O T A T I O N   F O R   T R U T H   V A L U E   A S S I G N M E N T S 
%-------------------------------------------------------------------------
%

% Default truth value
\newcommand{\truthval}{\nu}
\newcommand{\truthvalalt}{\mu}

% Default truth value assignments
\newcommand{\tvastd}{{\ensuremath{\alpha}}}
\newcommand{\tvaalt}{{\ensuremath{\beta}}}
\newcommand{\tvaalpha}{{\ensuremath{\alpha}}}
\newcommand{\tvabeta}{{\ensuremath{\beta}}}

% Logic formula evaluated under truth value assignment
% \logeval{expression to evalue}{truth value assignment}
\newcommand{\logeval}[2]{#2 ( #1 )}
\newcommand{\logevalstd}[1]{\tvastd ( #1 )}
\newcommand{\logevalcompact}[2]{#2 \bigl( #1 \bigr)}
\newcommand{\logevalcompactstd}[1]{\tvastd ( #1 )}
\newcommand{\Logeval}[2]{#2 \bigl( #1 \bigr)}
\newcommand{\Logevalstd}[1]{\tvastd ( #1 )}

% Modified truth value assignments
%
% \fliptva{truth value assignment}{variable}
%\newcommand{\fliptva}[2]{\ensuremath{\mathrm{flip}_{#1}^{#2}}}

\newcommand{\modtva}[2]{\ensuremath{#1^{#2}}}

\newcommand{\tvaflipall}[3][\tvastd]{\modtva{#1}{{#2} = {#3}}}
\newcommand{\tvaflipsupertrue}[2][\tvastd]{\tvaflipall[#1]{#2}{1}}
\newcommand{\tvaflipfalse}[2][\tvastd]{\tvaflipall[#1]{#2}{0}}


%
% N O T A T I O N   F O R   F O R M U L A S ,   V A R I A B L E S   E T C 
%-------------------------------------------------------------------------
%

%
% DEFAULT FORMULAS
%

% ``Default'' formulas \fstd and \fvar
\newcommand{\fstd}{{\ensuremath{F}}}
\newcommand{\fvar}{{\ensuremath{G}}}
\newcommand{\falt}{\fvar}

% Maybe change to more explicit macros \formf, \formg, \formh
\newcommand{\formf}{\ensuremath{F}}
\newcommand{\formg}{\ensuremath{G}}
\newcommand{\formh}{\ensuremath{H}}

%
% EMPTY CLAUSE
%

\newcommand{\emptycl}{0}
\newcommand{\emptyclvar}{\ensuremath{\Lambda}}

% OBSOLETE -- REMOVE!
%    \newcommand{\varstd}{\varx}
%    \newcommand{\varalt}{\vary}
%    \newcommand{\varfirst}{\varx}
%    \newcommand{\varsecond}{\vary}
%    \newcommand{\varthird}{\varz}
%    \newcommand{\varfourth}{\varw}
%    \newcommand{\litstd}{\lita}
%    \newcommand{\litalt}{\litb}
%    \newcommand{\litfirst}{\lita}
%    \newcommand{\litsecond}{\litb}
%    \newcommand{\litthird}{\litc}
%    \newcommand{\litfourth}{\litd}
%    \newcommand{\clstd}{\clc}
%    \newcommand{\clalt}{\cld}
%    \newcommand{\clfirst}{\cla}
%    \newcommand{\clsecond}{\clb}
%    \newcommand{\clthird}{\clc}
%    \newcommand{\clfourth}{\cld}
%    \newcommand{\clauseset}{\clsc}
%    \newcommand{\clset}{\clsc}

%
% DEFAULT VARIABLES
%

\newcommand{\varx}{\ensuremath{x}}
\newcommand{\vary}{\ensuremath{y}}
\newcommand{\varz}{\ensuremath{z}}
\newcommand{\varw}{\ensuremath{w}}

%
% DEFAULT LITERALS
%

\newcommand{\lita}{\ensuremath{a}}
\newcommand{\litb}{\ensuremath{b}}
\newcommand{\litc}{\ensuremath{c}}
\newcommand{\litd}{\ensuremath{d}}

%
% DEFAULT CLAUSES
%

\newcommand{\cla}{\ensuremath{A}}
\newcommand{\clb}{\ensuremath{B}}
\newcommand{\clc}{\ensuremath{C}}
\newcommand{\cld}{\ensuremath{D}}
\newcommand{\cle}{\ensuremath{E}}

%
% DEFAULT CLAUSE SETS
%

\newcommand{\clausesetformat}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\clsc}{\clausesetformat{C}}
\newcommand{\clsd}{\clausesetformat{D}}
\newcommand{\clse}{\clausesetformat{E}}

% Commented out 070706 -- \terms is in conflict with STOC style file    
\newcommand{\termt}{\ensuremath{T}}
%    \newcommand{\terms}{\ensuremath{S}}

%
% DEFAULT k-DNF FORMULA SETS   
%

\newcommand{\formulasetformat}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\fsf}{\formulasetformat{F}}
\newcommand{\fsg}{\formulasetformat{G}}


%
% SETS OF VARIABLES / LITERALS IN FORMULA
%

\newcommand{\setsofvarsorlitlarge}[2]%
        {\mathit{#1}\left({#2}\right)}
\newcommand{\setsofvarsorlit}[2]%
        {\mathit{#1}({#2})}
\newcommand{\setsofvarsorlitcompact}[2]%
        {\mathit{#1}\bigl({#2}\bigr)}
\newcommand{\setsofvarsorlitsmall}[2]
        {\mathit{#1}({#2})}
\newcommand{\setsofvarsorlitlarger}[2]
        {\mathit{{#1}}\biggl({#2}\biggr)}
\newcommand{\setsofvarsorlitsup}[3]%
        {\mathit{#1}^{#2}({#3})}
\newcommand{\setsofvarsorlitsuplarge}[3]%
        {\mathit{#1}^{#2}\left({#3}\right)}
\newcommand{\setsofvarsorlitsupcompact}[3]%
        {\mathit{#1}^{#2}\bigl({#3}\bigr)}

% OBSOLETE (with \ensuremath)
%    \newcommand{\setsofvarsorlitlarge}[2]%
%            {\ensuremath{\mathit{#1}\left({#2}\right)}}
%    \newcommand{\setsofvarsorlit}[2]%
%            {\ensuremath{\mathit{#1}({#2})}}
%    \newcommand{\setsofvarsorlitcompact}[2]%
%            {\ensuremath{\mathit{#1}\bigl({#2}\bigr)}}
%    \newcommand{\setsofvarsorlitsmall}[2]
%            {\ensuremath{\mathit{#1}({#2})}}
%    \newcommand{\setsofvarsorlitlarger}[2]
%            {\ensuremath{\mathit{{#1}}\biggl({#2}\biggr)}}
%    \newcommand{\setsofvarsorlitsup}[3]%
%            {\ensuremath{\mathit{#1}^{#2}({#3})}}
%    \newcommand{\setsofvarsorlitsuplarge}[3]%
%            {\ensuremath{\mathit{#1}^{#2}\left({#3}\right)}}
%    \newcommand{\setsofvarsorlitsupcompact}[3]%
%            {\ensuremath{\mathit{#1}^{#2}\bigl({#3}\bigr)}}


% OBSOLETE NOTATION
\newcommand{\varslarge}[1]{\setsofvarsorlitlarge{Vars}{#1}}
\newcommand{\litlarge}[1]{\setsofvarsorlitlarge{Lit}{#1}}
\newcommand{\varscompact}[1]{\setsofvarsorlitcompact{Vars}{#1}}
\newcommand{\litcompact}[1]{\setsofvarsorlitcompact{Lit}{#1}}
\newcommand{\varssmall}[1]{\setsofvarsorlitsmall{Vars}{#1}}
\newcommand{\litsmall}[1]{\setsofvarsorlitsmall{Lit}{#1}}
\newcommand{\litlarger}[1]{\setsofvarsorlitlarger{Lit}{#1}}

% NEW NOTATION
\newcommand{\vars}[1]{\setsofvarsorlitsmall{Vars}{#1}}
\newcommand{\lit}[1]{\setsofvarsorlitsmall{Lit}{#1}}
\newcommand{\VARS}[1]{\setsofvarsorlitlarge{Vars}{#1}}
\newcommand{\LIT}[1]{\setsofvarsorlitlarge{Lit}{#1}}
\newcommand{\Vars}[1]{\setsofvarsorlitcompact{Vars}{#1}}
\newcommand{\Lit}[1]{\setsofvarsorlitcompact{Lit}{#1}}

\newcommand{\varsset}{\mathit{Vars}}
\newcommand{\litset}{\mathit{Lit}}

%
% Restrictions
%

\newcommand{\restr}{\ensuremath{\rho}}
\newcommand{\rstd}{\restr}

\newcommand{\minfalserestr}[1]{\restr (\lnot #1)}
\newcommand{\minfalserestrcompact}[1]{\restr \bigl(\lnot #1 \bigr)}

\newcommand{\onerestr}[3]{{\restrict{#1}{#2 = #3}}}
\newcommand{\onerestrstd}{\onerestr{\fstd}{\varx}{\truthval}}

\newcommand{\restrict}[2]{{\ensuremath{{#1\!\!\upharpoonright}_{#2}}}}
\newcommand{\restrictOld}[2]{{\ensuremath{{#1 |}_{#2}}}}
%    \newcommand{\restrict}[2]{{\ensuremath{{#1 |}_{#2}}}}
\newcommand{\restrictstd}{{\restrict{\fstd}{\restr}}}




%
% P R O O F   C O M P L E X I T Y   M E A S U R E S 
%---------------------------------------------------
%

%       size
%       length
%       width
%       depth       OBSOLETE, REMOVED
%
% \xxx:         symbol for measurement
% \xxxofarg:    measurement of formulas, derivations etc
% \xxxref:      measurement of refutation       
% \xxxtree:     measurement of tree refutation
% \xxxderiv:    measurement of (general) derivation
%
% Commands \xxxof are not used to avoid conflict with mathtools package
%
% OBSOLETE:
% \xxxform:     measurement of formulas, derivations etc
%

\newcommand{\measstd}[1][]{\genericmeasure{M}{#1}}
\newcommand{\measstdof}[2][]{\genericform{{M}_{#1}}{#2}}

%
% NB! Do not touch these ``generic'' definitions unless you know
% *exactly* what you are doing!
%

\newcommand{\derivabbrev}[2]{\bigl( #1 \vdash #2 \bigr)}
\newcommand{\derivabbrevsmall}[2]{( #1 \vdash #2 )}
\newcommand{\derivabbrevcompact}[2]{\bigl( #1 \vdash #2 \bigr)}
\newcommand{\refutabbrev}[1]{\derivabbrev{#1}{\falsenum}}
\newcommand{\refutabbrevsmall}[1]{\derivabbrevsmall{#1}{\falsenum}}
\newcommand{\refutabbrevcompact}[1]{\derivabbrevcompact{#1}{\falsenum}}

\newcommand{\genericmeasure}[2]{{\mathit{#1}}_{#2}}
\newcommand{\genericform}[2]{\mathit{#1}\bigl( #2 \bigr)}
\newcommand{\genericformsmall}[2]{\mathit{#1}( #2 )}
\newcommand{\genericformcompact}[2]{\mathit{#1}\bigl( #2 \bigr)}
\newcommand{\genericref}[3]{{\mathit{#1}}_{#2}\refutabbrev{#3}}
\newcommand{\genericrefsmall}[3]%
    {{\mathit{#1}}_{#2}\refutabbrevsmall{#3}}
\newcommand{\genericrefcompact}[3]%
    {{\mathit{#1}}_{#2}\refutabbrevcompact{#3}}
\newcommand{\genericderiv}[4]%
    {{\mathit{#1}}_{#2}\derivabbrev{#3}{#4}}
\newcommand{\genericderivsmall}[4]%
    {{\mathit{#1}}_{#2}\derivabbrevsmall{#3}{#4}}
\newcommand{\genericderivcompact}[4]%
    {{\mathit{#1}}_{#2}\derivabbrevcompact{#3}{#4}}
\newcommand{\generictaut}[3]%
    {{\mathit{#1}}_{#2}\derivabbrev{}{#3}}
\newcommand{\generictautcompact}[3]%
    {{\mathit{#1}}_{#2}\derivabbrevcompact{}{#3}}
\newcommand{\generictautsmall}[3]%
    {{\mathit{#1}}_{#2}\derivabbrevsmall{}{#3}}
%    
%    \newcommand{\genericmeasure}[2]{\ensuremath{{\mathit{#1}}_{#2}}}
%    \newcommand{\genericform}[2]{\ensuremath{\mathit{#1}\bigl( #2 \bigr)}}
%    \newcommand{\genericformsmall}[2]{\ensuremath{\mathit{#1}( #2 )}}
%    \newcommand{\genericformcompact}[2]{\ensuremath{\mathit{#1}\bigl( #2 \bigr)}}
%    \newcommand{\genericref}[3]{\ensuremath{\mathit{#1}}_{#2}\refutabbrev{#3}}
%    \newcommand{\genericrefsmall}[3]%
%        {\ensuremath{{\mathit{#1}}_{#2}\refutabbrevsmall{#3}}}
%    \newcommand{\genericrefcompact}[3]%
%        {\ensuremath{{\mathit{#1}}_{#2}\refutabbrevcompact{#3}}}
%    \newcommand{\genericderiv}[4]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrev{#3}{#4}}}
%    \newcommand{\genericderivsmall}[4]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrevsmall{#3}{#4}}}
%    \newcommand{\genericderivcompact}[4]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrevcompact{#3}{#4}}}
%    \newcommand{\generictaut}[3]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrev{}{#3}}}
%    \newcommand{\generictautcompact}[3]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrevcompact{}{#3}}}
%    \newcommand{\generictautsmall}[3]%
%        {\ensuremath{{\mathit{#1}}_{#2}\derivabbrevsmall{}{#3}}}

% SIZE: OBSOLETE NOTATION
\newcommand{\size}[1][]{\genericmeasure{S}{#1}}
\newcommand{\sizeofsmall}[1]{\genericformsmall{S}{#1}}
\newcommand{\sizeofcompact}[1]{\genericformcompact{S}{#1}}

% SIZE: NEW NOTATION
\newcommand{\sizestd}{{\size}}
\newcommand{\sizeofarg}[1]{\genericformsmall{S}{#1}}
\newcommand{\Sizeofarg}[1]{\genericformcompact{S}{#1}}
\newcommand{\sizeref}[2][]{\genericrefsmall{S}{#1}{#2}}
\newcommand{\sizetaut}[2][]{\generictautsmall{S}{#1}{#2}}

% LENGTH: OBSOLETE NOTATION
\newcommand{\length}[1][]{\genericmeasure{L}{#1}}
\newcommand{\lengthofcompact}[1]{\genericformcompact{L}{#1}}
\newcommand{\lengthofsmall}[1]{\genericformsmall{L}{#1}}
\newcommand{\lengthrefsmall}[2][]{\genericrefsmall{L}{#1}{#2}}
\newcommand{\lengthtaut}[2][]{\generictaut{L}{#1}{#2}}
\newcommand{\lengthtautcompact}[2][]{\generictautcompact{L}{#1}{#2}}
\newcommand{\lengthtautsmall}[2][]{\generictautsmall{L}{#1}{#2}}
\newcommand{\lengthderivsmall}[3][]{\genericderivsmall{L}{#1}{#2}{#3}}

% LENGTH: NEW NOTATION
\newcommand{\lengthstd}{\length}
\newcommand{\lengthofarg}[1]{\genericformsmall{L}{#1}}
\newcommand{\Lengthofarg}[1]{\genericformcompact{L}{#1}}
\newcommand{\lengthref}[2][]{\genericrefsmall{L}{#1}{#2}}
\newcommand{\Lengthref}[2][]{\genericrefcompact{L}{#1}{#2}}
\newcommand{\lengthderiv}[3][]{\genericderivsmall{L}{#1}{#2}{#3}}
\newcommand{\Lengthderiv}[3][]{\genericderivcompact{L}{#1}{#2}{#3}}

% WIDTH: OBSOLETE NOTATION
\newcommand{\width}[1][]{\genericmeasure{W}{#1}}
\newcommand{\widthofsmall}[2][]{\genericformsmall{W_{#1}}{#2}}
\newcommand{\widthofcompact}[2][]{\genericformcompact{W_{#1}}{#2}}
\newcommand{\widthrefsmall}[2][]{\genericrefsmall{W}{#1}{#2}}
\newcommand{\widthderivsmall}[3][]{\genericderivsmall{W}{#1}{#2}{#3}}

% WIDTH: NEW NOTATION
% standard width denoted with small letter somewhat inconsequentially
\newcommand{\widthstd}{\ensuremath{w}} 

%
% \widthof is a conflict with the calc package
%
\newcommand{\widthofarg}[2][]{\genericformsmall{W_{#1}}{#2}}
\newcommand{\Widthofarg}[2][]{\genericformcompact{W_{#1}}{#2}}
\newcommand{\widthref}[2][]{\genericrefsmall{W}{#1}{#2}}
\newcommand{\Widthref}[2][]{\genericrefcompact{W}{#1}{#2}}
\newcommand{\widthderiv}[3][]{\genericderivsmall{W}{#1}{#2}{#3}}
\newcommand{\Widthderiv}[3][]{\genericderivcompact{W}{#1}{#2}{#3}}

%
% DEPTH MEASURE FROM MASTER'S THESIS---NOT USED ANYMORE
%
% Also, \depthof is a conflict with the calc package
%    \newcommand{\depthof}[2][]{\genericform{D_{#1}}{#2}}
%    \newcommand{\depthref}[2][]{\genericref{D}{#1}{#2}}
%    \newcommand{\depthtaut}[2][]{\generictaut{D}{#1}{#2}}
%

% TOTAL SPACE
\newcommand{\totspaceof}[1]{\genericformsmall{TotSp}{#1}}
\newcommand{\Totspaceof}[1]{\genericformcompact{TotSp}{#1}}
\newcommand{\totspaceref}[2][]{\genericrefsmall{TotSp}{#1}{#2}}
\newcommand{\Totspaceref}[2][]{\genericrefcompact{TotSp}{#1}{#2}}
\newcommand{\totspacederiv}[3][]{\genericderivsmall{TotSp}{#1}{#2}{#3}}
\newcommand{\Totspacederiv}[3][]{\genericderivcompact{TotSp}{#1}{#2}{#3}}

% CLAUSE SPACE: OBSOLETE NOTATION
\newcommand{\clspace}[1][]{\genericmeasure{Sp}{#1}}
\newcommand{\clspaceofsmall}[1]{\genericformsmall{Sp}{#1}}
\newcommand{\clspaceofcompact}[1]{\genericformcompact{Sp}{#1}}
\newcommand{\clspacerefsmall}[2][]{\genericrefsmall{Sp}{#1}{#2}}
\newcommand{\clspacerefcompact}[2][]{\genericrefcompact{Sp}{#1}{#2}}
\newcommand{\clspacederivsmall}[3][]{\genericderivsmall{Sp}{#1}{#2}{#3}}
\newcommand{\clspacetaut}[2][]{\generictaut{Sp}{#1}{#2}}

% CLAUSE SPACE: NEW NOTATION
\newcommand{\clspacestd}{{\clspace}}
\newcommand{\clspaceof}[2][]{\genericformsmall{Sp_{#1}}{#2}}
\newcommand{\Clspaceof}[2][]{\genericformcompact{Sp_{#1}}{#2}}
\newcommand{\clspaceref}[2][]{\genericrefsmall{Sp}{#1}{#2}}
\newcommand{\Clspaceref}[2][]{\genericrefcompact{Sp}{#1}{#2}}
\newcommand{\clspacederiv}[3][]{\genericderivsmall{Sp}{#1}{#2}{#3}}
\newcommand{\Clspacederiv}[3][]{\genericderivcompact{Sp}{#1}{#2}{#3}}

% VARIABLE SPACE: OBSOLETE NOTATION
\newcommand{\varspace}[1][]{\genericmeasure{VarSp}{#1}}
\newcommand{\varspaceofsmall}[1]{\genericformsmall{VarSp}{#1}}
\newcommand{\varspaceofcompact}[1]{\genericformcompact{VarSp}{#1}}
\newcommand{\varspacerefsmall}[2][]{\genericrefsmall{VarSp}{#1}{#2}}
\newcommand{\varspacerefcompact}[2][]{\genericrefcompact{VarSp}{#1}{#2}}
\newcommand{\varspacetaut}[2][]{\generictaut{VarSp}{#1}{#2}}

% VARIABLE SPACE: NEW NOTATION
\newcommand{\varspacestd}{{\varspace}}
\newcommand{\varspaceof}[1]{\genericformsmall{VarSp}{#1}}
\newcommand{\Varspaceof}[1]{\genericformcompact{VarSp}{#1}}
\newcommand{\varspaceref}[2][]{\genericrefsmall{VarSp}{#1}{#2}}
\newcommand{\Varspaceref}[2][]{\genericrefcompact{VarSp}{#1}{#2}}
\newcommand{\varspacederiv}[3][]{\genericderivsmall{VarSp}{#1}{#2}{#3}}
\newcommand{\Varspacederiv}[3][]{\genericderivcompact{VarSp}{#1}{#2}{#3}}


%
% ( S T A N D A R D )   P E B B L E   G A M E S 
%-----------------------------------------------
%

\newcommand{\formulaformat}[1]{\ensuremath{\mathit{#1}}}
\renewcommand{\formulaformat}[1]{\mathit{#1}}

% Format of pebble configurations 
\newcommand{\formatconfiguration}[1]{\mathbb{#1}}

% Format of pebbling strategies (or just ``pebblings'')
\newcommand{\formatpebblingstrategy}[1]{\mathcal{#1}}

% Transitions between configurations
\newcommand{\transitionarrow}{\rightsquigarrow}
\newcommand{\pebcfgtransition}[2]%
    {\ensuremath{#1 \transitionarrow #2}}
\newcommand{\pebcfgtransitionsqueeze}[2]%
    {#1 \! \transitionarrow \! #2}

% ``Default'' pebbling strategy
\newcommand{\pebbling}[1][P]{\formatpebblingstrategy{#1}}

% ``Default'' pebble configuration
\newcommand{\pconf}[1][P]{\formatconfiguration{#1}}

% Format of pebbling prices and space/cost of configurations
%    \newcommand{\formatpebblingprice}[1]{\text{\textit{#1}}}
%    \newcommand{\formatpebblingprice}[1]{\text{\textsc{#1}}}
\newcommand{\formatpebblingprice}[1]{\text{\textsl{\textsf{#1}}}}

\newcommand{\pebblingprice}[1]{\formatpebblingprice{Peb}(#1)}
\newcommand{\Pebblingprice}[1]%
    {\formatpebblingprice{Peb}\bigl(#1\bigr)}
\newcommand{\pebblingpricecompact}[1]%   OBSOLETE
    {\formatpebblingprice{Peb}\bigl(#1\bigr)}
\newcommand{\bwpebblingprice}[1]{\formatpebblingprice{BW-Peb}(#1)}
\newcommand{\Bwpebblingprice}[1]%
    {\formatpebblingprice{BW-Peb}\bigl(#1\bigr)}
\newcommand{\bwpebblingpricecompact}[1]%   OBSOLETE
    {\formatpebblingprice{BW-Peb}\bigl(#1\bigr)}

% Terminology and notation added in Nov 2008 for persistent pebblings
% (when black pebbles remain on all sinks) and visiting pebblings
% (when graphs is empty at the end of the pebbling)

\newcommand{\persistentpebadj}{persistent\xspace}
\newcommand{\persistentlypebadv}{persistently\xspace}
\newcommand{\visitingpebadj}{visiting\xspace}

\newcommand{\Persistentpebadj}{Persistent\xspace}
\newcommand{\Persistentlypebadv}{Persistently\xspace}
\newcommand{\Visitingpebadj}{Visiting\xspace}

%    \newcommand{\pebpersistentsymbol}{z}
\newcommand{\pebpersistentsymbol}{\bullet}
\newcommand{\pebvisitingsymbol}{\emptyset}

\newcommand{\bwpebpricepersistent}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebpersistentsymbol}(#1)}
\newcommand{\Bwpebpricepersistent}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebpersistentsymbol}\bigl(#1\bigr)}
\newcommand{\bwpebpricevisiting}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebvisitingsymbol}(#1)}
\newcommand{\Bwpebpricevisiting}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebvisitingsymbol}\bigl(#1\bigr)}

\newcommand{\pebpricepersistent}[1]%
    {\formatpebblingprice{Peb}^{\pebpersistentsymbol}(#1)}
\newcommand{\Pebpricepersistent}[1]%
    {\formatpebblingprice{Peb}^{\pebpersistentsymbol}\bigl(#1\bigr)}
\newcommand{\pebpricevisiting}[1]%
    {\formatpebblingprice{Peb}^{\pebvisitingsymbol}(#1)}
\newcommand{\Pebpricevisiting}[1]%
    {\formatpebblingprice{Peb}^{\pebvisitingsymbol}\bigl(#1\bigr)}

% OBSOLETE TERMINOLOGY
\newcommand{\bwpebblingpriceempty}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebvisitingsymbol}(#1)}
\newcommand{\bwpebblingpriceemptycompact}[1]%
    {\formatpebblingprice{BW-Peb}^{\pebvisitingsymbol}\bigl(#1\bigr)}

% Time of last move in pebblings or resolution derivations
\newcommand{\stoptime}{\tau}
% Time of some fixed move in pebblings or resolution derivations
\newcommand{\fixedtime}{\sigma}
% Time of start time in conditional pebbling
\newcommand{\starttime}{\sigma}

%
% Use the terminology "time" and "space" to measure number of
% moves and  pebbles in a pebbling. Phase out the concept of
% "cost". -- Nov 6, 2008 
%

\newcommand{\pebspace}[1]{\formatpebblingprice{space} ( #1 )}
\newcommand{\Pebspace}[1]{\formatpebblingprice{space} \bigl( #1 \bigr)}
\newcommand{\PEBSPACE}[1]{\formatpebblingprice{space} \left( #1 \right)}
\newcommand{\pebtime}[1]{\formatpebblingprice{time} ( #1 )}
\newcommand{\Pebtime}[1]{\formatpebblingprice{time} \bigl( #1 \bigr)}
\newcommand{\PEBTIME}[1]{\formatpebblingprice{time} \left( #1 \right)}

\newcommand{\pebcost}[1]{\formatpebblingprice{cost} ( #1 )}
\newcommand{\pebcostcompact}[1]{\formatpebblingprice{cost} \bigl( #1 \bigr)}
\newcommand{\pebcostsmall}[1]{\formatpebblingprice{cost} ( #1 )}


%
% F O R M U L A   F A M I L I E S 
%---------------------------------
%

%
% PEBBLING FORMULAS
%

\newcommand{\pebcontr}[2][G]{\ensuremath{\formulaformat{Peb}^{#2}_{#1}}}
\newcommand{\pebblingcontr}[2][G]{\pebcontr[#1]{#2}}

\newcommand{\pebdeg}{\ensuremath{d}}

\newcommand{\pebax}[2][\pebdeg]{\ensuremath{\formulaformat{Ax}^{#1} (#2)}}
\newcommand{\pebaxcompact}[2]%
        [\pebdeg]{\ensuremath{\formulaformat{Ax}^{#1} \bigl(#2 \bigr)}}

\newcommand{\varspeb}[1]{\setsofvarsorlitsup{Vars}{\pebdeg}{#1}}
\newcommand{\varspebcompact}[1]{\setsofvarsorlitsupcompact{Vars}{\pebdeg}{#1}}
\newcommand{\Varspeb}[1]{\setsofvarsorlitsupcompact{Vars}{\pebdeg}{#1}}

\newcommand{\pqrxvar}[6]%
    {\ensuremath{\stdnot{\varx({#1})}_{#2} \lor \stdnot{\varx({#3})}_{#4} \lor % 
    \sourceclausexvar[#6]{#5}}}
\newcommand{\pqrstdxvar}{\pqrxvar{p}{i}{q}{j}{r}{l}}

\newcommand{\pqr}[6]%
    {\ensuremath{\stdnot{#1}_{#2} \lor \stdnot{#3}_{#4} \lor % 
    \sourceclausenodisplay[#6]{#5}}}
\newcommand{\pqrstd}{\pqr{p}{i}{q}{j}{r}{l}}
\newcommand{\pqrall}[6]%
        {\setdescrcompact
        {\pqr{#1}{#2}{#3}{#4}{#5}{#6}}{#2,#4 \in \intnfirst{\pebdeg}}}
\newcommand{\pqrallstd}%
        {\setdescrcompact{\pqrstd}{i,j \in \intnfirst{\pebdeg}}}

\newcommand{\sourceclausexvar}[2][n]%
        {\Lor_{#1 = 1}^{\pebdeg} \varx({#2})_{#1}}
\newcommand{\subsourceclausexvar}[3][n]%
        {\Lor_{#1 = {#2}}^{\pebdeg} \varx({#3})_{#1}}
\newcommand{\targetclausexvar}[1][n]{\sourceclausexvar[#1]{z}}

\newcommand{\sourceclausexvarnodisplay}[2][n]%
        {\textstyle \Lor_{#1 = 1}^{\pebdeg} \varx({#2})_{#1}}

\newcommand{\sourceclause}[2][n]{\Lor_{#1 = 1}^{\pebdeg} #2_{#1}}
\newcommand{\subsourceclause}[3][n]{\Lor_{#1 = #2}^{\pebdeg} #3_{#1}}
\newcommand{\targetclause}[1][n]{\sourceclause[#1]{z}}

\newcommand{\sourceclausenodisplay}[2][n]%
        {\textstyle \Lor_{#1 = 1}^{\pebdeg} #2_{#1}}
\newcommand{\targetclausenodisplay}[1][n]{\sourceclausenodisplay[#1]{z}}

\newcommand{\sourceclausesuff}[2][n]{\Lor_{#1 \in \intnfirst{\pebdeg}} #2_{#1}}
\newcommand{\targetclausesuff}[1][n]{\sourceclausesuff[#1]{z}}

%
% TSEITIN FORMULAS
%

\newcommand{\tseitinform}{Tseitin formula\xspace}
\newcommand{\TSEITINFORM}{Tseitin Formula\xspace}
\newcommand{\tseitinnot}[2]{\ensuremath{\formulaformat{T}_{#1,#2}}}
\newcommand{\tseitinparity}[2]{\ensuremath{\formulaformat{PARITY}_{#1,#2}}}

%
% DENSE LINEAR ORDER FORMULAS
%

\newcommand{\dloform}{dense linear order principle\xspace}
\newcommand{\Dloform}{Dense linear order principle\xspace}
\newcommand{\DLOFORM}{Dense Linear Order Principle\xspace}
\newcommand{\dlonot}[1]{\ensuremath{\formulaformat{DLO}_{#1}}}
\newcommand{\extdlonot}[1]
    {\ensuremath{\extendedversion{\formulaformat{DLO}}_{#1}}}

%
% MINIMAL ELEMENT PRINCIPLE FORMULAS
%

\newcommand{\mepform}{minimal element principle\xspace}
\newcommand{\Mepform}{Minimal element principle\xspace}
\newcommand{\MEPFORM}{Minimal Element Principle\xspace}
\newcommand{\mepnot}[1]{\ensuremath{\formulaformat{MEP}_{#1}}}

\newcommand{\relativisation}[1]%
    {\ensuremath{\formulaformat{Rel}\bigl(#1 \bigr)}}

%
% PIGEONHOLE PRINCIPLE FORMULAS
%

\newcommand{\php}{pigeonhole principle\xspace}
%    \newcommand{\PHP}{\textit{PHP}\xspace}
\newcommand{\PHPform}{PHP~formula\xspace}
\newcommand{\PHPnot}[2]{\ensuremath{\formulaformat{PHP}^{#1}_{#2}}}
%    \newcommand{\PHPnot}[2]{\ensuremath{\formulaformat{PHP}_{#1}^{#2}}}
\newcommand{\extPHPnot}[2]
    {\ensuremath{\extendedversion{\formulaformat{PHP}}^{#1}_{#2}}}
\newcommand{\OntoPHPnot}[2]{\ensuremath{%
        \text{\formulaformat{Onto}-\formulaformat{PHP}}^{#1}_{#2}}}
\newcommand{\FPHPnot}[2]{\ensuremath{\formulaformat{FPHP}^{#1}_{#2}}}
\newcommand{\OntoFPHPnot}[2]{\ensuremath{%
        \text{\formulaformat{Onto}-\formulaformat{FPHP}}^{#1}_{#2}}}

\newcommand{\graphPHPform}{graph PHP formula\xspace}
\newcommand{\GraphPHPform}{Graph PHP formula\xspace}
\newcommand{\GraphPHPnot}[1][G]{\ensuremath{\formulaformat{PHP}_{#1}}}
\newcommand{\GraphFPHPnot}[1][G]{\ensuremath{\formulaformat{FPHP}_{#1}}}
\newcommand{\GraphOntoPHPnot}[1][G]{\ensuremath{%
        \text{\formulaformat{Onto}-\formulaformat{PHP}}_{#1}}}
\newcommand{\GraphOntoFPHPnot}[1][G]{\ensuremath{%
        \text{\formulaformat{Onto}-\formulaformat{FPHP}}_{#1}}}
\newcommand{\PHPstd}{\PHPnot{n+1}{n}}

% pigeonclause: pigeon i goes into some hole
% hole clause: pigeons i_1 and i_2 don't both go into hole j
% function clause: pigeon i doesn't go into holes j_1 and j_2
% onto clause: hole j gets some pigeon
\newcommand{\pigeonclause}[1]{\ensuremath{P_{#1}}}
\newcommand{\holeclause}[3]{\ensuremath{H_{#1,#2}^{#3}}}
\newcommand{\functionclause}[3]{\ensuremath{F_{#1}^{#2,#3}}}
\newcommand{\ontoclause}[1]{\ensuremath{S^{#1}}}

%
% CONTRADICTORY MATRIX FORMULAS
%

\newcommand{\Cmform}{Contradictory matrix formula\xspace}
\newcommand{\cmform}{contradictory matrix formula\xspace}
\newcommand{\cmnot}[2]{\ensuremath{\formulaformat{CM}_{#1,#2}}}
\newcommand{\cmnotstd}{\cmnot{n}{m}}

%
% GRAPH TAUTOLOGY FORMULAS
%

\newcommand{\gtform}{graph tautology formula\xspace}
\newcommand{\Gtform}{Graph tautology formula\xspace}
\newcommand{\gtnot}[1]{\ensuremath{\formulaformat{GT}_{#1}}}
\newcommand{\extgtnot}[1]
    {\ensuremath{\extendedversion{\formulaformat{GT}}_{#1}}}
\newcommand{\gttr}[1]{\ensuremath{A_{#1}}}
\newcommand{\gttrcl}[3]{\ensuremath{A \bigl( #1, #2, #3 \bigr)}}
\newcommand{\gttrclstd}{\gttrcl{i}{j}{k}}
\newcommand{\gtas}[1]{\ensuremath{B_{#1}}}
\newcommand{\gtascl}[2]{\ensuremath{B \bigl( #1, #2 \bigr)}}
\newcommand{\gtasclstd}{\gtascl{i}{j}}
\newcommand{\gtns}[1]{\ensuremath{C_{#1}}}
\newcommand{\gtnscl}[2]{\ensuremath{C_{#1} \bigl( #2 \bigr)}}
\newcommand{\gtnsclstd}{\gtnscl{n}{j}}

%
% RAMSEY FORMULAS    
%

\newcommand{\Ramseyform}{Ramsey formula\xspace}
\newcommand{\Ramseynot}[2]{\ensuremath{\formulaformat{RAM}^{#1}_{#2}}}

%
% EXTENDED VERSION (STRONG NONDETERMINISTIC EXTENSION) OF FORMULA
%

\newcommand{\extendedversion}[1]{\widetilde{#1}}



==> paperoutline.tex <==
\ifthenelse{\boolean{maybeIEEE}}
{In the rest of this paper, 
  we outline the main ideas in the proofs of our results in
  \refsec{sec:outline-proofs}
  and then  discuss some remaining open problems in
  \refsec{sec:concluding-remarks}.
  We refer to 
  \cite{Nordstrom10RelativeStrengthECCC}
  for missing formal definitions and full proofs.
}
{\subsection{Organization of 
  %    the Rest of 
  This Paper}

\ifthenelse{\boolean{confversionflag}}	   
{% CONFERENCE VERSION
  In
  \refsec{sec:outline-proofs}
  we outline the main ideas in the proofs of our results, and
  \refsec{sec:concluding-remarks}
  discusses  some remaining open problems.
  \Refsecapp{sec:preliminaries}
  contains  formal preliminaries. 
  \Refsecapp{sec:labelled-pebblings-proofs}
  proves our claims about the limited type of black-white pebblings
  that can be  simulated by resolution, and in
  \refsecapp{sec:bounded-labelled-pebblings}
  we show that there are such limited pebblings for some interesting
  graph families.
  In
  \refsecapp{sec:carlson-savage-proofs},
  we discuss the graphs exhibiting our new pebbling trade-off results,
  and show how different parameter settings yield
  strong dual time-space trade-offs 
  with upper bounds for black pebbling and
  matching lower bounds for black-white pebbling.
}
{% FULL-LENGTH VERSION
  In              
  \refsec{sec:outline-proofs}
  we outline the main ideas behind our results,
  and
  \refsecapp{sec:preliminaries}
  provides all the necessary preliminaries for the formal proofs of
  these results given in the rest of the paper.
  \Refsecapp{sec:labelled-pebblings-proofs}
  proves our claims about the limited type of black-white pebblings
  that can be  simulated by resolution, and in
  \refsecapp{sec:bounded-labelled-pebblings}
  we show that there are such limited pebblings for some interesting
  graph families.
  In
  \refsecapp{sec:carlson-savage-proofs},
  we discuss the graphs exhibiting our new pebbling trade-off results,
  and show how different parameter settings yield
  strong dual time-space trade-offs 
  with upper bounds for black pebbling and
  matching lower bounds for black-white pebbling.
  We conclude in
  \refsec{sec:concluding-remarks}
  by discussing some remaining open problems.
}
}


==> tentativenotation.tex <==
%
% THIS FILE CONTAINS NEW, TENTATIVE NOTATION AND TERMINOLOGY
%
% It is intended to be merged into the files ``definitions.tex'' 
% and ``notationProofComplexity.tex'' at some later stage when things
% have stabilized.
%


%    
%  ADAPTING OLD TERMINOLOGY  
%

\renewcommand{\lpebblingtext}{labelled pebbling\xspace}
\newcommand{\Lpebblingtext}{Labelled pebbling\xspace}
\renewcommand{\LPEBBLINGTEXT}{Labelled Pebbling\xspace}

\newcommand{\alpebblingtext}{a labelled pebbling\xspace}
\newcommand{\Alpebblingtext}{A labelled pebbling\xspace}

\renewcommand{\lpebblegame}{labelled pebble game\xspace}
\newcommand{\Lpebblegame}{Labelled pebble game\xspace}
\newcommand{\LPEBBLEGAME}{Labelled Pebble Game\xspace}

\newcommand{\bpblackparam}{m}
\newcommand{\bpwhiteparam}{S}

\newcommand{\nsboundedpebblingfull}[2]{$({#1},{#2})$-bounded \lpebblingtext}
\newcommand{\nsboundedpebbling}[2]{$({#1},{#2})$-bounded pebbling\xspace}
\newcommand{\boundedpebblingtext}{bounded pebbling\xspace}
\newcommand{\boundedlabelledpebblingtext}{bounded labelled pebbling\xspace}
\newcommand{\boundedpebblingfulltext}{bounded \lpebblingtext}



%
% MISCELLANEOUS
%

% A "sink pebbling" is a pebbling that touches all sinks.
\newcommand{\sinkpebblingtext}{sink pebbling\xspace}
\newcommand{\Sinkpebblingtext}{Sink pebbling\xspace}

% Sources and sinks of DAG
\newcommand{\sourcestd}{s}
\newcommand{\sinkstd}{z}
\newcommand{\sourcesetstd}{S}
\newcommand{\sinksetstd}{Z}
\newcommand{\sourcesof}[1]{S({#1})}
\newcommand{\sinksof}[1]{Z({#1})}

% Notation for pebbling interval
\newcommand{\pebint}[2]{\intclop{#1}{#2}}

% Terminology for essential pebble placements
\newcommand{\pebessential}{essential\xspace}
\newcommand{\Pebessential}{Essential\xspace}
\newcommand{\pebnonessential}{non-essential\xspace}
\newcommand{\Pebnonessential}{Non-essential\xspace}

% Parameter for # vertices of DAG
% (or # vertices to within constant factor)
\newcommand{\nvertices}{n}

% Parameter related to the size of a DAG, but not the size itself
% (if so, \nvertices would be used)
\newcommand{\sizerelatedparam}{m}

% ``Level parameter'' for DAG, such as depth of recursion (Carlson-Savage)
% or number of copies of sub-DAG (Lengauer-Tarjan)
\newcommand{\levelparam}{r}

% Parameter for indegree of dag
\newcommand{\indegreedag}{\ell}

% Parameter for depth of dag
\newcommand{\depthdag}{d}

% Parameter for space
\newcommand{\spacestd}{s}
\newcommand{\spacealt}{r}


%
% NOTATION NEEDED FOR LOUI'S UPPER BOUND PROOFS
%

\newcommand{\edgesfromto}[2]{\edges{#1,#2}}
\newcommand{\Edgesfromto}[2]{\Edges{#1,#2}}
\newcommand{\overlap}[1]{\formatfunctiontonumbers{io}({#1})}
\newcommand{\Overlap}[1]{\formatfunctiontonumbers{io}\bigl({#1}\bigr)}


%
% GRAPH FAMILIES
%
% Note that \Pi denotes pyramids and T (binary) trees
% Greek letter \Upsilon is not used for any DAGs
% Other upper-case greek letters are already used for other notation
%

% graph copy index---should the copy index G^i in the ith copy
% of the graph G in a construction be G^i or G^{(i)}?
\newcommand{\graphcopyindex}[1]{(#1)}

% Unfolding of graph
\newcommand{\unfold}[1]{\formatfunctiontoset{unfold}(#1)}
\newcommand{\unfoldingtext}{unfolding\xspace}
\newcommand{\unfoldtext}{unfold\xspace}
\newcommand{\Unfoldingtext}{Unfolding\xspace}
\newcommand{\Unfoldtext}{Unfold\xspace}

% "Single-sink version" of DAG (i.e. connecting all sinks into minimal
% tree to get single sink but same pebbling properties
\newcommand{\singlesinkdagtext}{single-sink DAG\xspace}
\newcommand{\Singlesinkdagtext}{Single-sink DAG\xspace}
\newcommand{\SINGLESINKDAGTEXT}{Single-Sink DAG\xspace}

\newcommand{\multisinkdagtext}{multi-sink DAG\xspace}
\newcommand{\Multisinkdagtext}{Multi-sink DAG\xspace}
\newcommand{\MULTISINKDAGTEXT}{Multi-Sink DAG\xspace}

\newcommand{\singlesinkversiontext}{single-sink version\xspace}
\newcommand{\Singlesinkversiontext}{Single-sink version\xspace}
\newcommand{\SINGLESINKVERSIONTEXT}{Single-Sink Version\xspace}
\newcommand{\singlesinkversion}[1]{\widehat{#1}}

% Superconcentrator
\newcommand{\supconcparam}{N}
\newcommand{\scparam}{\supconcparam}
\newcommand{\nsupconctext}[1]{\ensuremath{#1}-super\-concen\-trator\xspace}
\newcommand{\nsupconctextstd}{\nsupconctext{\supconcparam}}
\newcommand{\supconcnot}[2][]%
    {\ifthenelse{\equal{#1}{}}
    {\mathit{SC}_{#2}}
    {\mathit{SC}^{\graphcopyindex{#1}}_{#2}}}

% Carlson-Savage graphs:
\newcommand{\csnspines}{c}   % # spines in DAG
\newcommand{\csrec}{\levelparam}       % level of recursion in definition

\newcommand{\csdag}[2]{\Gamma({#1},{#2})}
%    \newcommand{\csdag}[2]{\Gamma^{#1}_{#2}}
\newcommand{\csdagstd}{\csdag{\csnspines}{\csrec}}
\newcommand{\csdagorig}[2]{\Gamma^*({#1},{#2})}
\newcommand{\csdagorigstd}{\csdagorig{\csnspines}{\csrec}}

\newcommand{\cssink}[1][]{\gamma_{#1}}
\newcommand{\cspyrsink}[1][]{z_{#1}}
\newcommand{\csspinevertex}[2]{{v[#1]}_{#2}}
%    \newcommand{\csspinevertex}[2]{v^{(#1)}_{#2}}
\newcommand{\cspebsurplus}{\spacestd}
\newcommand{\csconstant}{K}   % generic constant in proof
\newcommand{\csfunc}{g}   % arbitrarily slowly growing function
\newcommand{\csspine}{Q}
\newcommand{\cssection}{R}

% Permutation and bit reversal DAGs:
%bitrev{m}{i}: m-bit reversal of integer i < 2^m
\newcommand{\permstd}{\pi}              % standard permutation notation
\newcommand{\perminv}[1]{#1^{-1}}     % inverted permutation
\newcommand{\perminvstd}{\perminv{\pi}} % standard inverted permutation
\newcommand{\permnelems}{\nvertices}    % # elements to permute

% bit reversal permutation 
\newcommand{\bitrevop}{\formatfunctiontonumbers{rev}}
\newcommand{\bitrevopnbits}[1]{\bitrevop_{#1}}
\newcommand{\bitrev}[2]{\bitrevop_{#1}({#2})}
\newcommand{\brnbits}{\sizerelatedparam} 
\newcommand{\sppower}{r}

%    \newcommand{\permdag}[2]{\Delta^{#1}_{#2}}
\newcommand{\permdag}[2]{\Delta({#1},{#2})}
\newcommand{\permdagstd}{\permdag{\permnelems}{\permstd}}
\newcommand{\brdag}[1]{\permdag{#1}{\bitrevop}}

% Notation for chunks in bit reversal DAG proof
% \chunk{phase}{stage}
\newcommand{\chunk}[2]{C^{#1}_{#2}}


% Gilbert-Tarjan 1978
\newcommand{\gtdag}[2][]                
    {\ifthenelse{\equal{#1}{}}
    {\Xi({#2})}
    {\Xi^{\graphcopyindex{#1}}({#2})}}
\newcommand{\Gtdag}[2][]                
    {\ifthenelse{\equal{#1}{}}
    {\Xi \bigl({#2}\bigr)}
    {\Xi^{\graphcopyindex{#1}}\bigl({#2}\bigr)}}
%    \newcommand{\gtdag}[1]{\Upsilon_{#1})}
\newcommand{\gtsupconc}[2][]
    {\ifthenelse{\equal{#1}{}}
    {C({#2})}
    {C^{\graphcopyindex{#1}}({#2})}}

\newcommand{\gtcpnum}{c}

\newcommand{\gtmparam}[1]{M(#1)}
%    \newcommand{\gtmparam}[1]{m(#1)}

% first the graph index (i.e. ''recursion number''), then the vertex index
\newcommand{\gtsource}[3][]%
    {\ifthenelse{\equal{#1}{}}
     {\sourcestd_{#2}[#3]}
     {\sourcestd^{\graphcopyindex{#1}}_{#2}[#3]}}
\newcommand{\gtsink}[3][]%
    {\ifthenelse{\equal{#1}{}}
     {\sinkstd_{#2}[#3]}
     {\sinkstd^{\graphcopyindex{#1}}_{#2}[#3]}}
\newcommand{\scsource}[3][]%
    {\ifthenelse{\equal{#1}{}}
      {x_{#2}[#3]}
      {x^{\graphcopyindex{#1}}_{#2}[#3]}}
\newcommand{\scsink}[3][]%
    {\ifthenelse{\equal{#1}{}}
      {y_{#2}[#3]}
      {y^{\graphcopyindex{#1}}_{#2}[#3]}}



% Lengauer-Tarjan stacks of superconcentrators DAG (Sec 4)
\newcommand{\ltsupconcsize}{\sizerelatedparam}
\newcommand{\ltncopies}{\levelparam}
%    \newcommand{\ltsscdag}[2]{\Phi^{#1}_{#2}}
\newcommand{\ltsscdag}[2]{\Phi({#1},{#2})}
\newcommand{\ltsscdagstd}{\ltsscdag{\ltsupconcsize}{\ltncopies}}

\newcommand{\ltconstant}{K}   % generic constant in proof

% Lengauer-Tarjan exponential trade-offs DAG (Sec 5)
%    \newcommand{\ltexpdag}[2]{\Psi^{#1}_{#2}}
\newcommand{\ltexpdag}[2]{\Psi({#1},{#2})}

% \ksquadnot is the first [Kalyanasundaram-Schnitger 91] graph with 
% quadratic separation between black and black-white pebbling.
% \ksquadblock is the building block in this graph.
%
% \kspoly is the second [Kalyanasundaram-Schnitger 91] graph with 
% weaker separation but polynomial size.
% \kspolyblock is the building block in this graph.
%
% \ksncols is the number of columns in the meshes (p in the paper)
% \ksreclevel is the recursion level of the construction (j in the paper)
% \ksnrgraphs is the number of R-subgraphs (k in the paper)
% \ksnblocks is the number of blocks in the lower bound proof
% \kscol<x> are indices of particular columns in the proof
% \ksint are pebbling time intervals in the proof
% \kscol<x> are indices used for columns
% \ksslicec<x> are indices used for slices (boxes in KS91) corresponding to 
%    the columns
% \ksslicenot is the notation for a slice
% \ks[ab]nrows are the number of rows in the meshes in the second graph 
% (remains to be calculated after writing down the proof)
%
% \ksmeshtext is how the mesh structure should be named
%
% NB! Order of parameters for the graphs:
%
%    \ksquadnot{\ksncols}{\ksreclevel}
%    \kspolynot{\ksncols}{\ksreclevel}{\ksnrgraphs}
% 

\newcommand{\ksncols}{p}
\newcommand{\ksreclevel}{q}   
\newcommand{\ksnrgraphs}{k}
\newcommand{\ksnblocks}{m}
\newcommand{\ksint}{I}

\newcommand{\kscolc}{c}
\newcommand{\kscold}{d}
\newcommand{\kscole}{e}
\newcommand{\kscolf}{f}
\newcommand{\ksslicec}{c^*}
\newcommand{\kssliced}{d^*}
\newcommand{\ksslicee}{e^*}
\newcommand{\ksslicef}{f^*}

\newcommand{\ksslicenot}[2]{\formatfunctiontoset{slice}({#1}, {#2})}
\newcommand{\ksslicenotstd}{\ksslicenot{\ksnblocks + 1}{j}}

\newcommand{\ksbnrows}{(\ksncols + 1)^2}
\newcommand{\ksanrows}{(\ksncols + 1)^3}

\newcommand{\ksmeshtext}{spiral mesh\xspace}
\newcommand{\Ksmeshtext}{Spiral mesh\xspace}

\newcommand{\ksquadletter}{K}

\newcommand{\ksquadnot}[3][]%
  {\ifthenelse{\equal{#1}{}}
    {\ksquadletter}
    {\ksquadletter^{\graphcopyindex{#1}}}
    ({#2}, {#3})}
  
\newcommand{\kspolyletter}{\Lambda}
\newcommand{\kspolyauxgraph}{\kspolyletter'}

\newcommand{\kspolynot}[4][]%
  {\ifthenelse{\equal{#1}{}}
    {\kspolyletter}
    {\kspolyletter^{\graphcopyindex{#1}}}
    ({#2}, {#3}, {#4})}

\newcommand{\ksquadblockletter}{M}

\newcommand{\ksquadblock}[3][]%
  {\ifthenelse{\equal{#1}{}}
    {\ksquadblockletter}
    {\ksquadblockletter^{\graphcopyindex{#1}}}
    ({#2}, {#3})}
  
\newcommand{\kspolyblockletter}{N}

\newcommand{\kspolyblock}[4][]%
  {\ifthenelse{\equal{#1}{}}
    {\kspolyblockletter}
    {\kspolyblockletter^{\graphcopyindex{#1}}}
    ({#2}, {#3}, {#4})}

\newcommand{\ksquadnotnblocks}[4][]{\ksquadnot[#1]{#2}{#3}[#4]}

\newcommand{\ksquadnotnblocksext}[3]%
    {\ksquadletter^{+\ksbeforegraphletter} ({#1}, {#2})[#3]}
  
\newcommand{\kspolynotnblocks}[5][]{\kspolynot[#1]{#2}{#3}{#4}[#5]}

\newcommand{\kspolynotnblocksext}[4]%
    {\kspolyletter^{+\ksbeforegraphletter} ({#1}, {#2}, {#3})[#4]}
  

\newcommand{\ksquadnotstd}{\ksquadnot{\ksncols}{\ksreclevel}}
\newcommand{\ksquadblockstd}[1][]{\ksquadblock[#1]{\ksncols}{\ksreclevel}}
\newcommand{\ksquadnotnblocksstd}%
    {\ksquadnotnblocks{\ksncols}{\ksreclevel}{\ksnblocks}}
\newcommand{\ksquadnotnblocksextstd}%
    {\ksquadnotnblocksext{\ksncols}{\ksreclevel}{\ksnblocks}}

\newcommand{\kspolynotstd}{\kspolynot{\ksncols}{\ksreclevel}{\ksnrgraphs}}
\newcommand{\kspolyblockstd}[1][]{\kspolyblock[#1]{\ksncols}{\ksreclevel}{\ksnrgraphs}}
\newcommand{\kspolynotnblocksstd}%   
    {\kspolynotnblocks{\ksncols}{\ksreclevel}{\ksnrgraphs}{\ksnblocks}}
\newcommand{\kspolynotnblocksextstd}%
    {\kspolynotnblocksext{\ksncols}{\ksreclevel}{\ksnrgraphs}{\ksnblocks}}


% \ksbeforev: vertices in line/mesh before recursive graph
% \ksafterv: vertices in line/mesh after recursively constructed main graph
% \ksfirstrowv: first row of vertices (in main graph)
% \kslastrowv: last row of vertices (in main graph)
% \ksrcolv: vertices in vertical lines to the right of main graph

\newcommand{\ksbeforev}[1][]%
    {\ifthenelse{\equal{#1}{}}{b}{b^{\graphcopyindex{#1}}}}
\newcommand{\ksafterv}[1][]%
    {\ifthenelse{\equal{#1}{}}{a}{a^{\graphcopyindex{#1}}}}
\newcommand{\ksfirstrowv}[1][]%
    {\ifthenelse{\equal{#1}{}}{f}{f^{\graphcopyindex{#1}}}}
\newcommand{\kslastrowv}[1][]%
    {\ifthenelse{\equal{#1}{}}{l}{l^{\graphcopyindex{#1}}}}
\newcommand{\ksrcolv}[1][]%
    {\ifthenelse{\equal{#1}{}}{r}{r^{\graphcopyindex{#1}}}}

% Adding sub- and superindices to the vertices

\newcommand{\ksbeforevindices}[2]{b_{#1, #2}}
\newcommand{\ksaftervindices}[2]{a_{#1, #2}}
\newcommand{\ksrcolvindices}[2]{r_{#1, #2}}

\newcommand{\ksbeforevindicescopy}[3]{b^{\graphcopyindex{#1}}_{#2, #3}}
\newcommand{\ksaftervindicescopy}[3]{a^{\graphcopyindex{#1}}_{#2, #3}}
\newcommand{\ksrcolvindicescopy}[3]{r^{\graphcopyindex{#1}}_{#2, #3}}

\newcommand{\ksbeforevcopy}[2]{b^{\graphcopyindex{#1}}_{#2}}
\newcommand{\ksaftervcopy}[2]{a^{\graphcopyindex{#1}}_{#2}}
\newcommand{\ksfirstrowvcopy}[2]{\ksfirstrowv[#1]_{#2}}
\newcommand{\kslastrowvcopy}[2]{\kslastrowv[#1]_{#2}}


\newcommand{\ksbeforegraphletter}{B}
\newcommand{\ksbeforegraph}[1][]%
    {\ifthenelse{\equal{#1}{}}{B}{B^{\graphcopyindex{#1}}}}
\newcommand{\ksaftergraph}[1][]%
  {\ifthenelse{\equal{#1}{}}{A}{A^{\graphcopyindex{#1}}}}
\newcommand{\ksrcolgraph}[1][]%
  {\ifthenelse{\equal{#1}{}}{R}{R^{\graphcopyindex{#1}}}}
\newcommand{\ksrcolgraphindex}[2][]%	   
    {\ifthenelse{\equal{#1}{}}{R_{#2}}{R^{\graphcopyindex{#1}}_{#2}}}

% \nrowsb: shorthand for # rows in B-graph
% \nrowsa: shorthand for # rows in A-graph

\newcommand{\nrowsb}{n_b}
\newcommand{\nrowsa}{n_a}

\newcommand{\ksnewgoalvertex}%
    {\ksaftervindicescopy{\ksnblocks+1}{n'}{\kscold}}

%
% NOTATION FOR ``PROJECTED CLAUSES''
%
%    \newcommand{\formatfunctiontoset}[1]{\mathit{#1}}

%Projected clauses
% \projcl[projected down on which formula]{clause set being projected}
\newcommand{\projcl}[2][\fstd]{\formatfunctiontoset{proj}_{#1}({#2})}

\newcommand{\projectionsubst}{projection\xspace}
\newcommand{\projectverb}{project\xspace}
\newcommand{\projectingverb}{projecting\xspace}
\newcommand{\projectedverb}{projected\xspace}
\newcommand{\projectsverb}{projects\xspace}
\newcommand{\Projectionsubst}{Projection\xspace}
\newcommand{\Projectverb}{Project\xspace}
\newcommand{\Projectedverb}{Projected\xspace}
\newcommand{\Projectsverb}{Projects\xspace}

%
% \Lorspecfuncproj[pebbling degree]{variable}{clause}{function}
% \Lorspecnotfuncproj[pebbling degree]{variable}{clause}{function}
% \witnessproj[function]{pos lit}{neg lit}{clause}
%
\newcommand{\Lorspecfuncproj}[4][\pebdeg]%
    {\Lor_{{#2} \in \clpospart{#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncproj}[4][\pebdeg]%
    {\Lor_{\olnot{#2} \in \clnegpart{#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
\newcommand{\witnessproj}[4][\funcpebc]%	   
    {\Lorspecfuncproj{#2}{#4}{#1} \lor \Lorspecnotfuncproj{#3}{#4}{#1}}

\newcommand{\Lorspecfuncprojnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{{#2} \in \clpospart{#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncprojnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{\olnot{#2} \in \clnegpart{#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
\newcommand{\witnessprojnodisplay}[4][\funcpebc]%	   
    {\Lorspecfuncprojnodisplay{#2}{#4}{#1} \lor \Lorspecnotfuncprojnodisplay{#3}{#4}{#1}}


%
% NOTATION FOR ``VARIABLE SUPPORT SIZE''
%
\newcommand{\suppsizetext}{variable support size\xspace}
\newcommand{\Suppsizetext}{Variable support size\xspace}
\newcommand{\SUPPSIZETEXT}{Variable Support Size\xspace}
\newcommand{\suppsizeshorttext}{support size\xspace}
\newcommand{\Suppsizeshorttext}{Support size\xspace}
\newcommand{\SUPPSIZESHORTTEXT}{Support Size\xspace}

\newcommand{\suppsizeof}[1]{\genericformsmall{SuppSize}{#1}}
\newcommand{\Suppsizeof}[1]{\genericformcompact{SuppSize}{#1}}
\newcommand{\suppsizeref}[2][]{\genericrefsmall{SuppSize}{#1}{#2}}
\newcommand{\Suppsizeref}[2][]{\genericrefcompact{SuppSize}{#1}{#2}}
\newcommand{\suppsizederiv}[3][]{\genericderivsmall{SuppSize}{#1}{#2}{#3}}
\newcommand{\Suppsizederiv}[3][]{\genericderivcompact{SuppSize}{#1}{#2}{#3}}



%
% NOTATION FOR ``SUBSTITUTION FORMULAS''
%

\newcommand{\clpospart}[1]{#1^{+}}
\newcommand{\clnegpart}[1]{#1^{-}}
%    \newcommand{\clpospart}[1]{{#1}^{+}}
%    \newcommand{\clnegpart}[1]{{#1}^{-}}


% Substitution formula
% \substform{CNF formula}{Boolean function}
\newcommand{\substform}[2]{{#1}[{#2}]}
\newcommand{\Substform}[2]{{#1}\bigl[{#2}\bigr]}

\newcommand{\substformtext}{substitution formula\xspace}
\newcommand{\Substformtext}{Substitution formula\xspace}
\newcommand{\SUBSTFORMTEXT}{Substitution Formula\xspace}

\newcommand{\fsubsttext}[1][{\funcpebc[\pebdeg]}]%
    {${#1}$-substitution\xspace}
\newcommand{\substformtextwithargs}[2]{\fsubsttext[#1] of ${#2}$\xspace}
%
% NOTATION FOR GENERALIZED PEBBLING CONTRADICTIONS
%

%     \pebcontrwithfunc[graph]{degree}{function}
\newcommand{\pebcontrwithfunc}[3][G]{\formulaformat{Peb}^{#2}_{#1}[{#3}]}

% WARNING This ``3-cnf-version-via-tilde'' macro might not work well in displayed mode
\newcommand{\extendedpebcontrwithfunc}[3][G]%
    {{\vphantom{\formulaformat{Peb}}\smash{\extendedversion{\formulaformat{Peb}}}}^{#2}_{#1}[{#3}]}
%    \newcommand{\extendedpebcontrwithfunc}[3][G]%
%        {\extendedversion{\formulaformat{Peb}}^{#2}_{#1}[{#3}]}


% Generic pebbling contradiction with default Boolean function 
% (defined below) assumed as function
%     \genericpebcontr[graph]{degree}
\newcommand{\genericpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\funcpebc}}

% Analogous commands for pebbling formulas, i.e., target axioms removed
\newcommand{\pebcontrwithfuncNT}[3][G]%
     {\dummystar\!\!\formulaformat{Peb}^{#2}_{#1}[{#3}]}
\newcommand{\genericpebcontrNT}[2][G]%
     {\pebcontrwithfuncNT[#1]{#2}{\funcpebc}}

% Default Boolean function used in generalized pebbling contradictions
%     \funcpebc[degree] ; default is subindex being empty
\newcommand{\funcpebc}[1][]{f_{#1}}
\newcommand{\notfuncpebc}[1][]{\lnot f_{#1}}

%
% NOTATION FOR ``CANONICAL REPRESENTATIONS'' OF FUNCTIONS AS CNFs
%

%     \clfunc{function}{applied on vars of which vertex}{pebbling degree}
%     \clnotfunc is representation of negated function
\newcommand{\clausesreprfunction}{\formatfunctiontoset{Cl}}
\newcommand{\clfunc}[3]{\clausesreprfunction[{#1}_{{#3}}({\varvec{#2}})]}
\newcommand{\clnotfunc}[3]{\clausesreprfunction[\lnot{#1}_{{#3}}({\varvec{#2}})]}
%     \clfuncstd[function, default assumed]{vertex}
\newcommand{\clfuncstd}[2][\funcpebc]{\clfunc{#1}{#2}{\pebdeg}}
\newcommand{\clnotfuncstd}[2][\funcpebc]{\clnotfunc{#1}{#2}{\pebdeg}}

%
% NOTATION FOR THE BOOLEAN FUNCTIONS THEMSELVES
%

\newcommand{\varvec}[1]{\vec{#1}}

% Writing out the function as taking a vector 
%     \specfuncwithvecarg[degree]{function}{vertex}
%     \specnotfuncwithvecarg is same thing for negated function
\newcommand{\specfuncwithvecarg}[3][\pebdeg]%
	   {{#2}_{#1}(\varvec{#3})}
\newcommand{\specnotfuncwithvecarg}[3][\pebdeg]%
	   {\lnot {#2}_{#1}(\varvec{#3})}

%     \funcwithvecarg is same thing, except assuming default function
\newcommand{\funcwithvecarg}[2][\pebdeg]%
           {\specfuncwithvecarg[{#1}]{\funcpebc}{#2}}
\newcommand{\notfuncwithvecarg}[2][\pebdeg]%
           {\specnotfuncwithvecarg[{#1}]{\funcpebc}{#2}}

%     \funcwithvecargstd assumes also standard vertex v
\newcommand{\funcwithvecargstd}%
	   {\funcwithvecarg[\pebdeg]{v}}
\newcommand{\notfuncwithvecargstd}%
	   {\notfuncwithvecarg[\pebdeg]{v}}

% Writing out the function as taking d arguments v_1, ..., v_d
%     \specfuncwithargspebcontr[degree]{function}{vertex}
%     \specnotfuncwithargspebcontr is same thing for negated function
\newcommand{\specfuncwithargspebcontr}[3][\pebdeg]%
	   {{#2}_{#1}({#3}_1, \ldots, {#3}_{\pebdeg})}
\newcommand{\specnotfuncwithargspebcontr}[3][\pebdeg]%
	   {\lnot {#2}_{#1}({#3}_1, \ldots, {#3}_{\pebdeg})}

%     \funcwithargspebcontr is same thing, except assuming default function
\newcommand{\funcwithargspebcontr}[2][\pebdeg]%
	   {{\funcpebc}_{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}
\newcommand{\notfuncwithargspebcontr}[2][\pebdeg]%
	   {\lnot {\funcpebc}_{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}

%     \funcwithargspebcontrstd assumes also standard vertex v
\newcommand{\funcwithargspebcontrstd}%
	   {\funcwithargspebcontr[\pebdeg]{v}}
\newcommand{\notfuncwithargspebcontrstd}%
	   {\notfuncwithargspebcontr[\pebdeg]{v}}

%
% NOTATION FOR ``WITNESS CLAUSES'' FOR BLACK AND WHITE PEBBLES
%

% Witness clauses (or really witness functions) for black and white pebbles 
% for generic pebbling contradictions with default function f
%     \Lorfunc[degree]{vertex}{ranging over which vertex set}
\newcommand{\Lorfunc}[3][\pebdeg]
    {\Lor_{{#2} \in {#3}} \funcwithargspebcontr[#1]{#2}}
\newcommand{\Lornotfunc}[3][\pebdeg]
    {\Lor_{{#2} \in {#3}} \notfuncwithargspebcontr[#1]{#2}}

% ``Witness clauses'' where the Boolean function can be specified
%     \Lorspecfunc[degree]{vertex}{ranging over vertex set}{Boolean function}
\newcommand{\Lorspecfunc}[4][\pebdeg]%
    {\Lor_{{#2} \in {#3}} \specfuncwithargspebcontr[#1]{#4}{#2}}
\newcommand{\Lorspecnotfunc}[4][\pebdeg]%
    {\Lor_{{#2} \in {#3}} \specnotfuncwithargspebcontr[#1]{#4}{#2}}

% ``Witness clauses'' with vector notation for variables
%     \Lorspecfunc[degree]{vertex}{ranging over vertex set}{Boolean function}
\newcommand{\Lorspecfuncvec}[4][\pebdeg]%
    {\Lor_{{#2} \in {#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncvec}[4][\pebdeg]%
    {\Lor_{{#2} \in {#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
\newcommand{\Lorspecfuncvecnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{{#2} \in {#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncvecnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{{#2} \in {#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
    
% Shorthand for the full ``witness'' for the fact that black pebbles on 
% some vertex set and  white pebbles on some other vertex set are induced
%     \witnessclauserp[function]{b-variable}{black set}{w-variable}{white set}
\newcommand{\witnessclauserp}[5][\funcpebc]%	   
    {\Lorspecfuncvec{#2}{#3}{#1} \lor \Lorspecnotfuncvec{#4}{#5}{#1}}
\newcommand{\witnessclauserpnodisplay}[5][\funcpebc]%	   
    {\Lorspecfuncvecnodisplay{#2}{#3}{#1} \lor \Lorspecnotfuncvecnodisplay{#4}{#5}{#1}}
%        {\Lorspecfunc{#2}{#3}{#1} \lor \Lorspecnotfunc{#4}{#5}{#1}}

% Standard witness for subconfiguration [B]<W>
\newcommand{\witnessclauserpstd}[1][\funcpebc]%
    {\witnessclauserp[#1]{b}{B}{w}{W}}

%
% NOTATION & TERMINOLOGY FOR BOOLEAN FUNCTIONS USED IN PEBBL CONTRADICTIONS
%

% ``Non-authoritarian'' function
\newcommand{\authoritarian}{authoritarian\xspace}
\newcommand{\Authoritarian}{Authoritarian\xspace}
\newcommand{\nonauthoritarian}{non-authoritarian\xspace}
\newcommand{\Nonauthoritarian}{Non-authoritarian\xspace}

% Notation for standard or-pebbling contradiction
\newcommand{\orpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\lor}}
\newcommand{\orpebpyramidcontr}[2][]{\orpebcontr[\Pi_{#1}]{#2}}

\newcommand{\orpebcontrtext}{OR-pebbling contradiction\xspace}

% Notation for k-true-variables-out-of-d function
% \ntrues is default parameter for number of true variables k
\newcommand{\ntrues}{k}
%    \ktrue[out of d, omitted by default]{# true variables}
\newcommand{\ktrue}[2][]{{#2}\text{\textit{-true}}_{#1}}
% Standard notation for k-true-out-of-d
\newcommand{\ktruestd}[1][]{\ktrue[#1]{\ntrues}}
% Notation for k-true-out-of-d when also specifying parameter variables
\newcommand{\ktruewithargs}[2]%
    {\ktrue[\pebdeg]{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}

% Notation and name for k-out-of-d pebbling contradictions
\newcommand{\ktruepebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\ktruestd{}}}
\newcommand{\ktruepebcontrtext}[1][\ntrues]%
    {${#1}$-true-pebbling contradiction\xspace}

% Notation and terminology for XOR-pebbling contradictions
\newcommand{\xorpebcontrtext}{XOR-pebbling contradiction\xspace}

\newcommand{\xorpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\xor}}
\newcommand{\xorbinarypebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\xor_2}}

%Notation for the XOR function itself
\renewcommand{\xor}{\oplus}
\newcommand{\Xor}{{\textstyle \bigoplus}}

% ``Witness clauses'' for XOR function for individual vertices
\newcommand{\xorvertex}[3][\pebdeg]{\Xor_{{#3}=1}^{#1} {#2}_{#3}}
\newcommand{\notxorvertex}[3][\pebdeg]{\lnot \Xor_{{#3}=1}^{#1} {#2}_{#3}}

% Complete ``witness clauses'' for sets of black and white pebbles for 
% XOR-pebbling contradictions
\newcommand{\Lornotxor}[3][i]%
    {\Lor_{{#2} \in {#3}}\notxorvertex{#2}{#1}}
\newcommand{\Lorxor}[3][i]%
    {\Lor_{{#2} \in {#3}}\xorvertex{#2}{#1}}

%
% OUR MODIFIED PEBBLE GAME: ``RESOLUTION-PEBBLING GAME''
%

% Shorthand name for the DAGs that we are studying
\newcommand{\Generalpebblingdag}{Single-sink fan-in~$2$ DAG\xspace}
\newcommand{\generalpebblingdag}{single-sink fan-in~$2$ DAG\xspace}

% The name of our modified pebble game
\newcommand{\respebgame}{resolution-pebbling game\xspace}
\newcommand{\Respebgame}{Resolution-pebbling game\xspace}
\newcommand{\RESPEBGAME}{Resolution-Pebbling Game\xspace}

\newcommand{\respebgameshort}{res-pebbling game\xspace}
\newcommand{\Respebgameahort}{Res-pebbling game\xspace}

% Name of pebblings in the game
\newcommand{\respebblingtext}{res-pebbling\xspace}
\newcommand{\Respebblingtext}{Res-pebbling\xspace}
\newcommand{\RESPEBBLINGTEXT}{Res-Pebbling\xspace}
\newcommand{\respebblinglongtext}{resolution-pebbling\xspace}
\newcommand{\Respebblinglongtext}{Resolution-pebbling\xspace}
\newcommand{\RESPEBBLINGLONGTEXT}{Resolution-Pebbling\xspace}

% Notation for a res-pebbling
\newcommand{\respebbling}[1][R]{\pebbling[#1]}
%    \newcommand{\respebbling}[1][P]{\pebbling[#1]}

% Notation for res-pebbling cost and price
\newcommand{\respebprice}[1]{\formatpebblingprice{Res-Peb}(#1)}
\newcommand{\Respebprice}[1]{\formatpebblingprice{Res-Peb}\bigl(#1\bigr)}

\newcommand{\respebcost}[1]{\formatpebblingprice{cost}( #1 )}


% Notation and terminology for subconfigurations 
% in the res-pebbling game
\newcommand{\rpsubconf}{subconfiguration\xspace}
\newcommand{\Rpsubconf}{Subconfiguration\xspace}

\newcommand{\rpsubconflong}{\respebblingtext subconfiguration\xspace}
\newcommand{\Rpsubconflong}{\Respebblingtext subconfiguration\xspace}

% \rpscnot is notation for subconfigurations [B]<W>
%     \rpscnot{black set}{white set}
%     \Rpscnot{black set}{white set} has larger delimiters
\newcommand{\rpscnot}[2]{[ {#1} ] \langle {#2} \rangle}
\newcommand{\Rpscnot}[2]{\big[ {#1} \big] \bigl\langle {#2} \bigr\rangle}

% Standard subconfiguration [B]<W>
\newcommand{\rpscnotstd}[1][]{\rpscnot{B_{#1}}{W_{#1}}}

% Notation and terminology for SETS of 
% subconfigurations in the res-pebbling game
\newcommand{\rpconftext}{\respebblingtext con\-fig\-u\-ra\-tion\xspace}
\newcommand{\Rpconftext}{\Respebblingtext con\-fig\-u\-ra\-tion\xspace}

\newcommand{\rpconf}[1][R]{\pconf[#1]}

% Notation for some special subconfigurations
%    \rpscrpq = [r]<p,q>
\newcommand{\rpscrpq}{\rpscnot{r}{p,q}}
%    \rpscintro{v} = [v]<pred(v)>
\newcommand{\rpscintro}[1]{\rpscnot{#1}{\prednode{#1}}}
%     \rpscuncondblack{v} =   [v]<empty set>
\newcommand{\rpscuncondblack}[1]{\rpscnot{#1}{\emptyset}}

% Notation for induced res-pebbling configurations
\newcommand{\rpinducedconf}[1]{\rpconf(#1)}

% Shorthand for induced configurations at times t-1 and t that keep
% recurring in the proofs
\newcommand{\rpinducedctminusone}{\rpinducedconf{\clsc_{t-1}}}
\newcommand{\rpinducedct}{\rpinducedconf{\clsc_{t}}}

% Notation for cost \leq # clauses proof
\newcommand{\allvertices}{V^*}
\newcommand{\matchingstd}{M}

%
% TENTATIVE NAMES OF RESOLUTION-PEBBLING MOVES
%
% (consistently described by using macros so that terminology can easily be 
% changed if need be)
%
% Names of macros reflect the names chosen in previous papers
% Actual macros right now insted try to give intuition for the correspondence 
% with resolution derivation steps
%

\newcommand{\rpintro}{download\xspace}
\newcommand{\rpanintro}{a download\xspace}
\newcommand{\Rpintro}{Download\xspace}
\newcommand{\Rpanintro}{A download\xspace}

\newcommand{\rpintroduce}{download\xspace}

\newcommand{\rpmerger}{resolution\xspace}
\newcommand{\rpamerger}{a resolution\xspace}
\newcommand{\Rpmerger}{Resolution\xspace}
\newcommand{\Rpamerger}{A resolution\xspace}

\newcommand{\rpmerge}{resolve\xspace}
\newcommand{\rpmerging}{resolving\xspace}

\newcommand{\rpinflation}{weakening\xspace}
\newcommand{\rpaninflation}{a weakening\xspace}
\newcommand{\Rpinflation}{Weakening\xspace}
\newcommand{\Rpaninflation}{A weakening\xspace}

\newcommand{\rpinflate}{weaken\xspace}
\newcommand{\rpinflated}{weakened\xspace}

\newcommand{\rperasure}{erasure\xspace}
\newcommand{\rpanerasure}{an erasure\xspace}
\newcommand{\Rperasure}{Erasure\xspace}
\newcommand{\Rpanerasure}{An erasure\xspace}



